Regularizing with Pseudo-Negatives for Continual Self-Supervised Learning

We introduce a novel Pseudo-Negative Regularization (PNR) framework for effective continual self-supervised learning (CSSL). Our PNR leverages pseudo-negatives obtained through model-based augmentation in a way that newly learned representations may not contradict what has been learned in the past. Specifically, for the InfoNCE-based contrastive learning methods, we define symmetric pseudo-negatives obtained from current and previous models and use them in both main and regularization loss terms. Furthermore, we extend this idea to non-contrastive learning methods which do not inherently rely on negatives. For these methods, a pseudo-negative is defined as the output from the previous model for a differently augmented version of the anchor sample and is asymmetrically applied to the regularization term. Extensive experimental results demonstrate that our PNR framework achieves state-of-the-art performance in representation learning during CSSL by effectively balancing the trade-off between plasticity and stability.

==> 3_method_prev.tex <==
\vspace{-0.1in}
\section{Main Method}
\subsection{Problem Setting}\label{sec:setting}
\noindent\textbf{Notations and preliminaries.}  \ \
We evaluate the quality of CSSL methods using the setting and data for continual supervised learning similarly as in \cite{(cassle)fini2022self}. Namely, let $t$ be the task index, where $t \in \{1, \dots, T\}$, and $T$ represents the maximum number of tasks. The input data and their corresponding true labels given at the $t$-th task are denoted by $ x \in \mathcal{X}_t$ and $y \in \mathcal{Y}_t$, respectively\footnote{For concreteness, we explicitly work with image data in this paper, but we note that our method is general and not confined to image modality.}. 
We assume each training dataset for task $t$ comprises 
$M$ supervised pairs, denoted as $\mathcal{D}_t = \{ (x_i, y_i)\}^{M}_{i=1}$, in which each pair is considered to be sampled from a joint distribution $p(\mathcal{X}_t, \mathcal{Y}_t)$.
Note in the case of continual supervised learning (CSL)~\citep{(cl_survey2)delange2021continual, (cil_survey)masana2020class}, both inputs and the labels are used, whereas in CSSL~\citep{(cassle)fini2022self,(continuity)madaan2022representational}, only input data are utilized for training, while the true labels are used only for the evaluation of the learned representations, such as linear probing or $k$-NN evaluation~\citep{(cassle)fini2022self, (repeval)cha2023objective}. 
We denote $h_{\theta_t}$ as the representation encoder (with parameter $\theta_t$) learned after task $t$ by a CSSL method. To evaluate the quality of $h_{\theta_{t}}$ via linear probing, we consider a classifier $f_{\Theta_{t}}= o_{\phi_{t}}\circ h_{\theta_{t}}$, in which $\Theta_t=(\theta_t,\phi_t)$ and $o_{\phi_{t}}$ is the linear output layer (with parameter $\phi_t$) on top of $h_{\theta_{t}}$. Then, only $o_{\phi_{t}}$ is supervised trained (with frozen $h_{\theta_{t}}$) using all the training dataset $\mathcal{D}_{1:t}$, including the labels, and the accuracy of resulting $f_{\Theta_{t}}$ becomes the proxy for the represenation quality. 


\noindent\textbf{Class-/Data-/Domain-incremental learning.}  \ \
We consider the three scenarios of continual learning as outlined in \cite{(CL_scenarios)van2019three, (cl_survey3)wang2023comprehensive, (cassle)fini2022self}. We use $k$ and $j$ to denote arbitrary task numbers, where $k,j\in \{1,\ldots,T\}$ and $k \neq j$. 
The first category is the \textit{class-incremental learning} (Class-IL), in which the $t$-th task's dataset consists of a unique set of classes for the input data, namely, $p(\mathcal{X}_k)\neq p(\mathcal{X}_j)$ and $\mathcal{Y}_k \cap \mathcal{Y}_j = \varnothing$.
The second category is \textit{domain-incremental learning} (Domain-IL), in which each dataset $\mathcal{D}_t$ has the same set of true labels but with different distribution on $\mathcal{X}_t$, denoted as $p(\mathcal{X}_k)\neq p(\mathcal{X}_j)$ but $\mathcal{Y}_k = \mathcal{Y}_j$.
In other words, each dataset in Domain-IL contains input images sampled from a different domain, but the corresponding set of true labels is the same as for other tasks.
Finally, we consider \textit{data-incremental learning} (Data-IL), in which a set of input images $\mathcal{X}_t$ is sampled from a single distribution, $p(\mathcal{X}_k) = p(\mathcal{X}_j)$, but $\mathcal{Y}_k = \mathcal{Y}_j$. 
To implement the Data-IL scenario in our experiments, we shuffled the entire dataset (such as ImageNet-100) and divided it into $T$ disjoint datasets.




\subsection{Motivation}\label{sec:motivation}

\noindent\textbf{Conventional loss form of continual learning}  \ \ 
We first reconsider the loss form, illustrated in Figure \ref{figure1:general_loss}, which is commonly employed by many state-of-the-art continual learning (CL) methods, except in cases where exemplar memory is utilized. 
Namely, when learning task $t$ with a model parameter $\Theta_t$, the conventional loss has the form as follows:
\begin{equation}
\mathcal{L}^{t}_{\mathrm{CL}}(\mathcal{D}_t, \Theta_t, \Theta_{t-1}) = \mathcal{L}_{\mathrm{single}}(\mathcal{D}_t, \Theta_t) + \lambda\cdot\mathcal{L}_{\mathrm{reg}}(\mathcal{D}_t, \Theta_t, \Theta_{t-1}),\label{eqn:general_cl}
\end{equation}
in which $\Theta_{t-1}$ represents the frozen model trained up to task $t-1$ and $\lambda$ denotes a regularization parameter that controls appropriate trade-off between the two loss terms.
\csm{The term $\mathcal{L}_{\mathrm{single}}$ represents the typical loss function utilized in single-task learning, such as cross-entropy, supervised contrastive loss ~\citep{(sup_contrastive)khosla2020supervised} or self-supervised learning loss~\citep{(moco)he2020momentum}.} This term clearly promotes \textit{plasticity} for the new task (task $t$) since it depends only on the current model $\Theta_{t}$ and $\mathcal{D}_t$. In addition, $\mathcal{L}_{\mathrm{reg}}$ represents a regularization term that is dedicated to increase \textit{stability}. Namely, since $\Theta_{t-1}$ is considered to contain knowledge of the previous tasks' dataset (\textit{i.e.}, $\mathcal{D}_{1:t-1}$) in the weight parameters, $\mathcal{L}_{\mathrm{reg}}$ is solely designed to maintain that knowledge to reduce forgetting while training $\Theta_t$ in various ways: such as direct weight level-regularization~\citep{(ewc)kirkpatrick2017overcoming}, knowledge distillation~\citep{(lwf)li2017learning} from $\Theta_{t-1}$ to $\Theta_{t}$, and model expansion term~\citep{(der)yan2021dynamically}.
\csm{It's worth noting that recent works on CSSL~\citep{(stream)hu2022how, (cassle)fini2022self, (continuity)madaan2022representational} also adopt a similar loss formulation as (\ref{eqn:general_cl}). In particular, CaSSLe~\citep{(cassle)fini2022self}, the current state-of-the-art method, introduces a novel and effective $\mathcal{L}_{\text{reg}}$ that easily integrates with various self-supervised learning methods, effectively mitigating catastrophic forgetting in learned representations during CSSL.}
% , such as Moco \citep{(moco)he2020momentum}, SimCLR \citep{(simclr)chen2020simple}, BYOL~\citep{(byol)grill2020bootstrap}, and BarlowTwins \citep{(barlow_twins)zbontar2021barlow}, etc.

Nevertheless, we contend that the utilization of such a conventional loss form may impose limitations on the achievement of more successful CSSL. This stems from the fact that while $\mathcal{L}_{\text{reg}}$ contributes to the preservation of previously acquired representations and the reduction of forgetting  , it may impede the acquisition of new representations from novel tasks. Furthermore, recent empirical findings, as highlighted in studies such as \citep{(repeval)cha2023objective, davari2022probing}, suggest that prioritizing \textit{stability} through regularization ($\mathcal{L}_{\text{reg}}$) may not necessarily result in learning improved representations even when higher accuracy is attained, thereby supporting this proposition.


\begin{figure}[t]
\vspace{-.1in}
\centering 
\subfigure[Conventional loss form of CL]
{\includegraphics[width=0.34\linewidth]{figures/fig1_a.pdf}
\label{figure1:general_loss}}
\subfigure[Lack of diversity of negative samples in CSSL]
{\includegraphics[width=0.64\linewidth]{figures/fig1_b.pdf}
\label{figure1:diversity}}
\vspace{-.15in}
\caption{Illustrations of motivation for our work. 
(a) Many of the CL algorithms combine a loss dedicated to learning a single current task and a regularizer that penalizes the deviation of the current model from the past.  
(b): In CSSL, negative samples are solely mined from the current task's data, resulting in significantly decreasing diversity of negative samples than the case of the joint SSL.}
\label{figure:fig1}
\vspace{-.2in}
 \end{figure}

\noindent\textbf{Low diversity of negative samples in CSSL}  \ \ 
In contrast to the prevailing research trend in CSSL, we assert that CSSL faces a critical challenge stemming from the \textit{limited diversity of negative samples} when compared to joint self-supervised learning (Joint SSL). 
\csm{The importance of negative samples in self-supervised contrastive learning has been extensively acknowledged, with studies demonstrating the benefits of incorporating a substantial number of diverse negative samples ~\citep{(infonce)oord2018representation,(contrastive_analysis)wang2020understanding, (simclr)chen2020simple, (selfsup_analysis)tao2022exploring} and selecting hard negatives ~\citep{(cont_hard_neg1)robinson2020contrastive,(cont_hard_neg2)kalantidis2020hard}. However, the issue of negative samples in the CSSL has remained unexplored until now.} In this regard, Figure \ref{figure1:diversity} highlights a fundamental problem: while Joint SSL allows for diverse negative sample selection, CSSL tends to exhibit significantly reduced diversity. Given the importance of negative samples, we believe that this decrease in diversity can be a key reason why self-supervised contrastive learning algorithms often yield less effective representations in CSSL scenarios, especially in terms of \textit{plasticity}.


% \csm{To tackle these new challenges, we pioneer the use of additional negative representations from both the $t$ and $t-1$ models to enhance the quality of learned representations during CSSL. Furthermore, we propose a simple but novel idea to apply these negative representations, not only to contrastive learning methods that leverage negatives ~\citep{(simclr)chen2020simple, (moco)he2020momentum} but also to conventional SSL methods that do not use negatives~\citep{(barlow_twins)zbontar2021barlow, (byol)grill2020bootstrap, (vicreg)bardes2022vicreg}.}



\subsection{Augmenting Negative Representations for Contrastive Learning Methods}\label{sec:method_contrastive} \ 

\begin{figure*}[h]
\vspace{-.05in}
\centering 
{\includegraphics[width=0.98\linewidth]{figures/fig2.pdf}}
\vspace{-.05in}
\caption{\csm{Graphical representation of learning with our proposed AugNeg loss. The blue dashed arrow represents the direction of the gradient update when training with the AugNeg loss, repelling from the negative sample embeddings of current/past models and attracting to the positive sample embeddings of the current/past models.}}
\vspace{-.2in}
\label{figure:recon_loss}
 \end{figure*}
 
Motivated by the two issues raised in the previous section, we propose a new form of loss functions tailored for CSSL. First, recalling the notation in Section \ref{sec:setting}, we note that only the encoder $h_{\theta_t}$ is trained during CSSL. Then, our Augmented Negatives (AugNeg) loss, devised for contrastive learning-based methods,  for learning from task $t$ has the following form
\begin{equation}
\mathcal{L}^{t}_{\text{AugNeg}}(\mathcal{D}_t, \theta_{t}, \theta_{t-1}) = \mathcal{L}_{\text{1}}(\mathcal{D}_t, \theta_{t}, \theta_{t-1}) + \mathcal{L}_{\text{2}}(\mathcal{D}_t, \theta_{t}, \theta_{t-1}).\label{eqn:recon}
\end{equation} 
While we will specify the two loss functions shortly, here, notice the symmetric dependence of them on $(\mathcal{D}_t,\theta_t,\theta_{t-1})$, which is in contrast to (\ref{eqn:general_cl}). As we show below, such symmetry enables our loss to promote finding inherent trade-off between the plasticity and stability without explicit control of a hyperparameter. 

\noindent\textbf{Model-based augmentation of negative representations.}  \ \ 
To address the issue depicted in Figure \ref{figure1:diversity} and based on the format of Equation (\ref{eqn:recon}), we propose 
to make use of augmented negative representations obtained from the both current and previous models \csm{during training task $t$}.
For given input data $x_i$ and encoder $h_{\theta_t}$, we denote  $z_{i, t} = \text{Proj}(h_{\theta_t}({x}_i)) \in \mathcal{R}^{D_P}$ and $\tilde{z}_{i, t} = \text{Pred}(z_{i, t}) \in \mathcal{R}^{D_P}$ as the normalized embeddings for the encoder of task $t$, in which ``Proj'' and ``Pred'' are the Projection~\citep{(simclr)chen2020simple} and Prediction~\citep{(cassle)fini2022self} layers, consisting of a multi-layer perceptron (MLP), respectively. Furthermore, we denote $z^{+}_{i,t}$ and $z^{-}_{i,t}$ as the embedding (obtained by $h_{\theta_t}$) of the \textit{positive} and \textit{negative} sample corresponding to the given $x_{i}$, respectively, and $\mathcal{N}_t(i)$ as the set of the negative embeddings for $x_i$. Then, both losses in (\ref{eqn:recon}) for the sample $x_i$ are defined as 
\begin{equation}
\mathcal{L}_{\text{1}}(x_i,\theta_t,\theta_{t-1}) = - {\mathrm{log}}\frac{\mathrm{exp}(z_{i, t} \cdot z^{+}_{i,t} / \tau)}{\sum_{z^{-}_{i,t}\in \mathcal{N}_t(i)}{\mathrm{exp}(z_{i, t} \cdot z^{-}_{i,t} / \tau) + {\sum_{z^{-}_{i,t-1}\in \mathcal{N}_{t-1}(i)}\mathrm{exp}(z_{i, t} \cdot z^{-}_{i,t-1} / \tau)}}}
\label{eqn:plasticity},\nonumber
\end{equation} 
and
\begin{equation}
\mathcal{L}_{\text{2}}(x_i,\theta_t,\theta_{t-1}) = - {\mathrm{log}}\frac{\mathrm{exp}(\tilde{z}_{i, t} \cdot z_{i,t-1} / \tau)}{\sum_{z^{-}_{i,t}\in \mathcal{N}_t(i)}{\mathrm{exp}(\tilde{z}_{i, t} \cdot z^{-}_{i,t} / \tau) + {\sum_{z^{-}_{i,t-1}\in \mathcal{N}_{t-1}(i)}\mathrm{exp}(\tilde{z}_{i, t} \cdot z^{-}_{i,t-1} / \tau)}}}\label{eqn:stability}.\nonumber
\end{equation} 
in which $\tau$ is a temperature parameter. 

Note these two losses are quite similar in form to InfoNCE~\citep{(infonce)oord2018representation}, but has a couple of key differences. Previous CL research, such as CaSSLe, $z_{i,t-1}$ was solely utilized for distilling previous knowledge (for better \textit{stability}).
In contrast to them, 
firstly, in $\mathcal{L}_{\text{1}}$, we use \textit{additional} negative embeddings in $\mathcal{N}_{t-1}(i)$ which are obtained from the previous model $h_{\theta_{t-1}}$. 
This addition of negative embeddings in $\mathcal{L}_{\text{1}}$ mitigates the issue of decreasing diversity of negative samples pointed out in Section \ref{sec:motivation}. Moreover, it compels the embedding of $x_i$ to be repelled not only from the negative embeddings of the current model but also from those of the previous model, hence, it fosters the acquisition of more distinctive representations. Secondly, in $\mathcal{L}_{\text{2}}$, which has the similar form of self-supervised distillation ~\citep{(cont_distill2)fang2021seed,(cont_distill1)tian2019contrastive}, we also use \textit{additional} negative embeddings in $\mathcal{N}_t(i)$. Such modification has an impact of putting additional constraint in distillation so that the representations from the past model are maintained in a way not to contradict with the representations of current model. Also, we introduce the ``Pred'' layer, as in \cite{(cassle)fini2022self}, to not hurt the plasticity by doing indirect distillation. 

Note that the denominators of the two loss functions are identical except for the ``Pred'' step in $\mathcal{L}_{\text{2}}$. 
Therefore, with the identical repelling negative embeddings, adding two losses will  result in achieving natural trade-off between plasticity and stability for learning the representation $z_{i,t}$. This intuition is depicted in Figure \ref{figure:recon_loss}. Namely, unlike in Figure \ref{figure1:general_loss}, both losses symmetrically consider the embeddings from current and previous models, and as shown in the rightmost hypersphere, the representation of $z_{i,t}$ gets attracted to $z_{i,t}^{+}$ and $z_{i,t-1}$ with the constraint that it is far from both $z_{i,t}^-$ and $z_{i,t-1}^-$. Thus, the new representation will be distinctive from the previous model (\textit{plasticity}) and carry over the old knowledge (\textit{stability}) in a way not to hurt the current model. 

 \csm{It is noteworthy that the AugNeg loss can be easily integrated into contrastive learning-based SSL methods like MoCo and SimCLR. The implemented loss function for them is presented in the Supplementary Materials. Also, 
in the Supplementary Materials, we provide more discussions and analyses, such as the gradient analysis for the proposed loss $\mathcal{L}_{\text{AugNeg}}$, the role of augmented negatives.}


\subsection{Extension to the Non-Contrastive Learning Methods}\label{sec:method_non_contrastive}
\csm{For SSL algorithms that do not utilize negatives (e.g., Barlow, BYOL and VICReg}), the core idea of AugNeg which utilizes model-based augmentation of negative representations cannot be directly applied.
However, we can apply the similar principle by adding an additional regularization term. For instance, consider a batch of input images denoted as \(x\), where distinct augmentations, denoted as \(A\) and \(B\), are applied, resulting in \(x^{A}\) and \(x^{B}\), respectively. 
Based on this, the loss function for the AugNeg loss s BYOL can be denoted as follows:
\begin{align}
\mathcal{L}^{t}_{\text{AugNeg, BYOL}}(x^{\text{A}}, x^{\text{B}}, \theta_{t}, \theta_{t-1}) = 
\|g_{\theta_t}(h_{\theta_t}(x^{\text{A}})) - {z_{\xi}}(x^{\text{B}})\|^2_2\label{eqn:byol} \\ +  
\|\text{Pred}(h_{\theta_t}(x^{\text{A}})) - h_{\theta_{t-1}}(x^{\text{A}})\|^2_2\label{eqn:cassle_byol} \\ -  
\|\text{Pred}(h_{\theta_t}(x^{\text{A}})) - h_{\theta_{t-1}}(x^{\text{B}})\|^2_2\label{eqn:augneg_byol}, 
\end{align}
where $q_{\theta_t}$ represents an MLP layer in BYOL, and $z_{\xi}$ corresponds to the target network obtained through momentum updates using $h_\theta$. 
Equation (\ref{eqn:byol}) and Equation (\ref{eqn:cassle_byol}) denotes the original loss function of BYOL and CaSSLe's distillation, respectively.
% Equation (\ref{eqn:byol}) maintains consistency with the self-supervised loss function used in the original BYOL. Equation (\ref{eqn:cassle_byol}) mirrors the approach employed in CaSSLe for distillation, which mitigates catastrophic forgetting in CSSL. 
Furthermore, \csm{Equation (\ref{eqn:augneg_byol}) is a newly devised regularization to enhance \textit{plasticity} by using negatives from the $t-1$ model.} Unlike Equation (\ref{eqn:cassle_byol}), where the outputs of models $t$ and $t-1$ task remain consistent when the same augmentation is applied, Equation (\ref{eqn:augneg_byol}) ensures that when different augmentations are applied, model $t$ produces different outputs from model $t-1$ (i.e., considering the output of model $t-1$ as negative samples). The justification for Equation (\ref{eqn:augneg_byol}) can be substantiated by the approach utilized in contrastive distillation of CaSSLe, where all samples with distinct augmentations (e.g., $2N$ samples) consider all samples except those with the same augmentation (e.g., $2N-1$ samples) as negative samples (See the Supplementary Materials for more details).
\csm{Note that the similar form of Equation \ref{eqn:augneg_byol} can be utilized for the case of AugNeg(VICReg) also. We believe that the above idea can similarly be applied to various SSL algorithms that do not explicitly involve negative samples through the addition of extra regularization. The implementation details for VICReg and Barlow are introduced in the Supplementary Materials.}

% where $q_{\theta_t}$ represents a MLP layer of BYOL, while $z_{\xi}$ corresponds to the target network obtained through momentum updates using $h_\theta$. 
% Equation (3) remains consistent with the self-supervised loss function employed in the original BYOL. 
% Equation (4) mirrors the implementation of CaSSLe~\cite{(cassle)fini2022self}'s distillation, which is employed to mitigate catastrophic forgetting in CSSL. Furthermore, Equation (5) introduces an additional regularization term. Unlike Equation (4), where the outputs of models $t$ and $t-1$ task remain consistent when the same augmentation is applied, Equation (5) ensures that, when different augmentations are applied, the model $t$ produces different outputs from the model $t-1$ (i.e., taking into account the output of the $t-1$ model as negative samples). 
% Also, the justification for Equation (5) can be substantiated by the approach utilized in CaSSLe for contrastive distillation between model t and t-1, where  considering all samples, except those with the same augmentation (e.g., 2N-1) as negative samples among all samples with distinct augmentations (e.g., 2N samples). 

% Similarly, we believe that our idea can be applied to various SSL algorithms that do not explicitly consider negative samples in the form of additional regularization. The implementation details of BarlowTwins are available in the Supplementary Materials. 

% \subsection{Discussion: the Role of Augmented Negative Representations}
% Incorporating augmented negative representations from the previous model (referred to as the $t-1$ model) aligns with SSL algorithms such as BYOL and MoCo, which leverage positive representations from a momentum encoder. This momentum encoder progressively enhances their representations by assimilating updates from the training encoder, thus contributing to the successful \textit{positive} representations for SSL. In contrast, in CSSL, the current task model (typically initialized as the $t-1$ model) is trained by leveraging information from the previous model. It's important to note that, while the previous model may have achieved adequate uniformity and alignment for the previous task dataset~\cite{(contrastive_analysis)wang2020understanding}, it may not exhibit the same characteristics when applied to a new task, as shown in Figure \ref{figure:recon_loss}. Therefore, in scenarios involving knowledge distillation (similar to CaSSLe~\cite{(cassle)fini2022self}), merely distilling the representations of samples from the current task dataset, such as representations of the same image with the same augmentation (\textit{e.g.}, Equation (4) and the numerator of $L_2$) may have a limitation to achieve a superior representation.

% In this regard, using augmented negative representations from the previous model can be considered as contributing to the informative additional \textit{negative} representations for CSSL. By additionally incorporating representations from both the models (\textit{e.g.,} the denominator of $L_1$ and $L_2$) or the previous model (\textit{e.g.,} Equation (5)) as supplementary negative representations, the newly trained model can learn superior and novel representations, taking into account both uniformity and alignment of not only the current but also previous model.



==> iclr2023/1_intro.tex <==
\section{Introduction}

Self-Supervised Learning (SSL) has recently emerged as a cost-efficient approach for training neural networks, eliminating the need for laborious data labelling~\citep{(ssl_survey)gui2023survey}. 
Specifically, the representations learned by recent SSL methods (\textit{e.g.,} MoCo~\citep{(moco)he2020momentum}, SimCLR~\citep{(simclr)chen2020simple},  BarlowTwins~\citep{(barlow_twins)zbontar2021barlow}, BYOL~\citep{(byol)grill2020bootstrap}, and {VICReg~\citep{(vicreg)bardes2022vicreg}})
are shown to have excellent quality, comparable to those learned from supervised learning. Despite such success, huge memory and computational complexities are the apparent bottlenecks for easily maintaining and updating the self-supervised learned models, {since they typically require large-scale unsupervised data, large mini-batch sizes, and numerous gradient update steps for training}. 
 
To that end, Continual Self-Supervised Learning (CSSL), in which the aim is to learn progressively improved representations from a sequence of unsupervised data, can be an efficient alternative to the high-cost, jointly trained self-supervised learning. With such motivation, several recent studies \citep{(continuity)madaan2022representational, (stream)hu2022how, (cassle)fini2022self} have considered the CSSL using various SSL methods and showed their effectiveness in maintaining representation continuity. Despite the positive results, we note that the core idea for those methods is mainly borrowed from the large body of continual learning research for supervised learning \citep{(cl_survey1)parisi2019continual, (cl_survey2)delange2021continual, (cl_survey3)wang2023comprehensive}. Namely, a typical supervised continual learning method can be generally described as employing a single-task loss term for the new task (\textit{e.g.,} cross-entropy or supervised contrastive loss~\citep{(sup_contrastive)khosla2020supervised}) together with a certain type of 
regularization (\textit{e.g.,} distillation-based~\citep{(lwf)li2017learning,(podnet)douillard2020podnet, (afc)kang2022class, (foster)wang2022foster, (co2l)cha2021co2l} or norm-based~\citep{(ewc)kirkpatrick2017overcoming, (MAS)aljundi2018memory, (AGS-CL)jung2020adaptive, (UCL)ahn2019uncertainty,(cpr)cha2021cpr} or replay-sample based terms \citep{(bic)wu2019large, (icarl)rebuffi2017icarl}) to prevent forgetting; the recent state-of-the-art CSSL methods simply follow that approach with \textit{self-supervised} loss terms \csmcm{(\textit{e.g.}, CaSSLe~\cite{(cassle)fini2022self})}.

In this regard, we raise an issue on the current CSSL approach; the efficacy of simply incorporating a regularization term into the existing self-supervised loss for achieving successful CSSL remains uncertain. Namely, typical regularization terms are essentially designed to maintain the representations of the previous model, but they may hinder the capability of learning better representations while learning from the new task \csmcm{(\textit{i.e., plasticity)}} ~\citep{(repeval)cha2023objective, kim2023stability}. 

\csm{To address these limitations, we propose a novel method called Pseudo-Negative Regularization (PNR) for CSSL, which utilizes \textit{pseudo-negatives} for each anchor of a given input, obtained by model-based augmentation. 
In the CSSL using various SSL methods, PNR defines different pseudo-negatives tailored for each contrastive and non-contrastive learning method, respectively.
Firstly, we consider the case of using InfoNCE-type contrastive loss~\cite{(infonce)oord2018representation}, such as SimCLR and MoCo, which explicitly leverages negative samples. 
\csmcm{We propose novel loss functions by modifying the ordinary InfoNCE loss and contrastive distillation~\cite{(cont_distill1)tian2019contrastive}, ensuring that the former considers negatives from the previous model and the latter includes negatives from the current model as the \csmcm{pseudo-negatives}.}
% In other words, the proposed loss functions consider the same set of the negatives from both the current and previous models at the same time. 
As a result, these loss functions ensure that newly acquired representations do not overlap with previously learned ones, enhancing \csmcm{\textit{plasticity}}. Moreover, they enable effective distillation of prior knowledge into the current model without interfering with the representations already learned by the current model, thereby improving overall \csmcm{\textit{stability}}. 
Second, we extend the idea of using pseudo-negatives to CSSL using non-contrastive learning methods like BYOL, BarlowTwins, and VICReg, which \csmcm{do not} explicitly employ negative samples in their original implementations. 
\csmcm{For this, we reevaluate the relationship between the anchor of the current model and the negatives from the previous model observed in the contrastive distillation}
Building on this relationship, we propose a novel regularization that defines the \csmcm{pseudo-negative} for the anchor from the current model as the output feature of the same image with different augmentations from the previous model. Our final loss function aims to minimize their similarity by incorporating this regularization alongside the existing distillation term for CSSL.
Finally, through extensive experiments, our proposed method not only achieves state-of-the-art performance in CSSL scenarios and downstream tasks but also shows both better \textit{stability} and \textit{plasticity}.}

% In summary, our core contributions are summarized as below:

% \begin{compactitem}
% \item \csm{We propose Pseudo-Negative Regularization (PNR) exclusively for CSSL, specifically tailored for each contrastive and non-contrastive learning SSL method.}
% \item \csm{To employ the PNR, we introduce novel loss functions based on InfoNCE and contrastive distillation for contrastive learning, and a novel regularization for non-contrastive learning.}
% \item \csm{We experimentally confirm that the proposed loss functions using pseudo negative achieves state-of-the-art performance acoss various CSSL scenarios and downstream tasks.}
% \end{compactitem}

==> iclr2023/2_related_work.tex <==
% \vspace{-0.1in}
\section{Related Work}


\noindent\textbf{Self-supervised representation learning} \ \
There have been several recent variations for Self-Supervised Learning (SSL)~\citep{(pretext1)alexey2016discriminative, (pretext2)doersch2015unsupervised, (denoising_autoencoder)vincent2010stacked, (colrization)zhang2016colorful, (cont_init)hadsell2006dimensionality, (simclr)chen2020simple, (moco)he2020momentum}.
Among those, 
{\textit{contrastive loss-based} methods have emerged as one of the leading approaches to learn discriminative representations~\citep{(cont_init)hadsell2006dimensionality, (infonce)oord2018representation}, in which the representations are learned by pulling the positive pairs together and pushing the negative samples apart.
Several efficient contrastive learning methods, like MoCo~\citep{(moco)he2020momentum,(mocov2)chen2020improved}, SimCLR~\citep{(simclr)chen2020simple}, have been proposed build on the InfoNCE loss~\citep{(infonce)oord2018representation}.}
Additionally, \textit{non-contrastive learning} methods, such as Barlow Twins~\citep{(barlow_twins)zbontar2021barlow}, BYOL~\citep{(byol)grill2020bootstrap} and {VICReg~\citep{(vicreg)bardes2022vicreg}, have been demonstrated to yield high-quality learned representations without \csmcm{using negative samples}.}

\noindent\textbf{Continual learning}  \ \
Continual learning (CL) is the process of acquiring new knowledge while retaining previously learned knowledge \citep{(cl_survey1)parisi2019continual, (cil_survey)masana2020class} from a sequence of tasks. 
To balance the trade-off between \textit{plasticity}, the ability to learn new tasks well, and \textit{stability}, the ability to retain  knowledge of previous tasks~\citep{(tradeoff)mermillod2013stability}, the {supervised} CL research has been proposed in several categories.
For more details, one can refer to ~\citep{(cl_survey3)wang2023comprehensive, (cl_survey2)delange2021continual}. 

\noindent\textbf{Continual Self-Supervised Learning}  \ \
Recently, there has been a growing interest in Continual Self-Supervised Learning (CSSL), as evidenced by several related researches \citep{(unsup_representation_cl)rao2019continual, (continuity)madaan2022representational, (stream)hu2022how, (cassle)fini2022self}. 
While all of them explore the possibility of using unsupervised datasets for CL, they differ in their perspectives.
\cite{(unsup_representation_cl)rao2019continual} is the first to introduce the concept of unsupervised continual learning and proposed a novel approach to learning class-discriminative representations without any knowledge of task identity.
\cite{(continuity)madaan2022representational} \csmcm{proposes a novel data augmentation method for CSSL} and first demonstrates that CSSL can outperform supervised CL algorithms in the task-incremental learning scenario.
Another study~\citep{(stream)hu2022how} focuses on the benefits of CSSL in large-scale datasets (\textit{e.g.}, ImageNet), demonstrating that a competitive pre-trained model can be obtained through CSSL.
\csmcm{The first significant regularization for CSSL was proposed by CaSSLe~\cite{(cassle)fini2022self}.
They devised a novel regularization that helps to overcome catastrophic forgetting in CSSL, achieving state-of-the-art performance in various scenarios without using exemplar memory.
After that, several papers have been published but they consider settings that are different from CaSSLe. C$^2$ASR~\citep{cheng2023contrastive} considers to use the exemplar memory and introduces both a novel loss function and exemplar sampling strategy.
\cite{yu2024evolve, tang2024kaizen, gomez2024plasticity} are tailored for semi-supervised learning scenarios and demonstrate superior performance in such cases. Additionally, \cite{yu2024evolve, gomez2024plasticity} are dynamic architecture-based algorithms where the model expands as the number of tasks grows.}


\csmcm{In this paper, we offer a few distinctive contributions compared to above mentioned related works. 
First, we identify shortcomings in the conventional regularization-based loss formulation for CSSL, such as CaSSLe. 
Second, we introduce a novel concept of pseudo-negatives and propose a new loss function that incorporates this concept, applicable to both contrastive and non-contrastive learning-based CSSL.}

% Second, we introduce two novel forms of a loss function, that leverage pseudo negative, applied to both contrastive and non-contrastive learning SSL methods, respectively. It's important to note that these proposed loss functions are specifically designed for CSSL, setting them apart from CaSSLe, which proposes the application of existing SSL methods for distillation, and C$^2$ASR, which utilizes exemplar memory for successful CSSL.


==> iclr2023/3_method.tex <==
\section{Problem Setting}\label{sec:setting}
\noindent\textbf{Notations and preliminaries.}  \ \
We evaluate the quality of CSSL methods using the setting and data as in \cite{(cassle)fini2022self}. Namely, let $t$ be the task index, where $t \in \{1, \dots, T\}$, and $T$ represent the maximum number of tasks. The input data and their corresponding true labels given at the $t$-th task are denoted by $ \bm x \in \mathcal{X}_t$ and $y \in \mathcal{Y}_t$, respectively\footnote{For concreteness, we explicitly work with image data in this paper, but we note that our method is general and not confined to image modality.}. 
Let $\mathcal{D}$ is the entire dataset. We assume each training dataset for task $t$ comprises 
$M$ supervised pairs, denoted as $\mathcal{D}_t = \{ (\bm x_i, y_i)\}^{M}_{i=1}$, in which each pair is considered to be sampled from a joint distribution $p(\mathcal{X}_t, \mathcal{Y}_t)$.
Note in the case of continual supervised learning (CSL)~\citep{(cl_survey2)delange2021continual, (cil_survey)masana2020class}, both inputs and the labels are used, whereas in CSSL~\citep{(cassle)fini2022self,(continuity)madaan2022representational}, only input data are utilized for training, while the true labels are used only for the evaluation of the learned representations, such as linear probing or $k$-NN evaluation~\citep{(cassle)fini2022self, (repeval)cha2023objective}. 
Let \csmcm{$m_{\bm \psi_{t}} \circ h_{\bm \theta_t} $  is the model consisting of the representation encoder (with parameter $\bm \theta_t$) and an MLP layer (with parameter $\bm \psi_{t}$) learned after task $t$.}
To evaluate the quality of $h_{\bm \theta_{t}}$ via linear probing, we consider a classifier $f_{\bm \Theta_{t}}= o_{\bm \phi_{t}}\circ h_{\bm \theta_{t}}$, in which $\bm \Theta_t=(\bm \theta_t,\bm \phi_t)$ and $o_{\bm \phi_{t}}$ is the linear output layer (with parameter $\bm \phi_t$) on top of $h_{\bm \theta_{t}}$. Then, only $o_{\bm \phi_{t}}$ is supervised trained (with frozen $h_{\bm \theta_{t}}$) using all the training dataset $\mathcal{D}_{1:t}$, including the labels, and the accuracy of resulting $f_{\bm \Theta_{t}}$ becomes the proxy for the representation quality. 


\noindent\textbf{Class-/Data-/Domain-incremental learning.}  \ \
We consider the three scenarios of continual learning as outlined in \cite{(CL_scenarios)van2019three, (cl_survey3)wang2023comprehensive, (cassle)fini2022self}. We use $k$ and $j$ to denote arbitrary task numbers, where $k,j\in \{1,\ldots,T\}$ and $k \neq j$. 
The first category is the \textit{class-incremental learning} (Class-IL), in which the $t$-th task's dataset consists of a unique set of classes for the input data, namely, $p(\mathcal{X}_k)\neq p(\mathcal{X}_j)$ and $\mathcal{Y}_k \cap \mathcal{Y}_j = \varnothing$.
The second category is \textit{domain-incremental learning} (Domain-IL), in which each dataset $\mathcal{D}_t$ has the same set of true labels but with different distribution on $\mathcal{X}_t$, denoted as $p(\mathcal{X}_k)\neq p(\mathcal{X}_j)$ but $\mathcal{Y}_k = \mathcal{Y}_j$.
In other words, each dataset in Domain-IL contains input images sampled from a different domain, but the corresponding set of true labels is the same as for other tasks.
Finally, we consider \textit{data-incremental learning} (Data-IL), in which a set of input images $\mathcal{X}_t$ is sampled from a single distribution, $p(\mathcal{X}_k) = p(\mathcal{X}_j)$, but $\mathcal{Y}_k = \mathcal{Y}_j$. 
To implement the Data-IL scenario in our experiments, we shuffle the entire dataset (such as ImageNet-100) and divide it into $T$ disjoint datasets.

\begin{figure}[t]
% \vspace{-.05in}
\centering 
{\includegraphics[width=0.95\linewidth]{figures/new_fig1.pdf}}
\vspace{-.05in}
\caption{The overview of using pseudo-negatives in CSSL with contrastive learning. Note that red dashed arrows denote the incorporation of the proposed \csmcm{pseudo-negatives}, which are output features from distinct models,  in each loss function.}
\vspace{-.15in}
\label{figure:motivation}
 \end{figure}

\section{Pseudo-Negative Regularization (PNR)}

\subsection{Motivation}\label{sec:motivation}
Several studies have been conducted with the aim of progressively improving the quality of representations learned by the encoder ($h_{\bm \theta_{t}}$) in CSSL. 
While it has been noted that simple fine-tuning using $D_t$ results in less severe forgetting compared to  supervised continual learning~\cite{(continuity)madaan2022representational, davari2022probing}, CaSSLe~\cite{(cassle)fini2022self} has achieved even more successful CSSL.
\csmcm{It introduces a novel regularization method based on existing SSL methods, using the output features of both the encoder at time $t$ and the encoder at time $t-1$, to overcome catastrophic forgetting in learned representations.}
Despite CaSSLe achieving promising results in various experiments, our motivation arises from the belief that incorporating \textit{pseudo-negatives} can lead to even more successful results. Consider an augmented image obtained by applying different augmentations to the input image $\bm x$, denoted by $\bm x^A$ and $\bm x^B$. 
% The output features of the $h_{\bm \theta_t}$ and $h_{\bm \theta_{t-1}}$ encoders 
\csmcm{The output features of the $m_{\bm \psi_{t}} \circ h_{\bm \theta_t} $ and $m_{\bm \psi_{t-1}} \circ h_{\bm \theta_t-1} $} 
for these augmented images are denoted by $\bm z^A_{t}$, $\bm z^B_{t}$, $\bm {z}^A_{t-1}$, and $\bm {z}^B_{t-1}$, respectively. 
In contrast to CaSSLe, our approach involves utilizing the output features of both the models as pseudo-negatives, as illustrated in Figure \ref{figure:motivation}. For this purpose, we propose a novel CSSL loss form for task $t$, defined as follows:
% \begin{equation}
% \begin{aligned}
% \mathcal{L}_{t}^{\text{CSSL}}(\bm x^A, \bm x^B; \bm \theta_t, \bm \theta_{t-1}) &= \mathcal{L}^{\text{SSL}^*}_1(z^A, z^B, \bar{z}^A, \bar{z}^B) \\ &+  \mathcal{L}^{\text{SSL}^*}_2(g(z^A), \bar{z}^A, z^A, z^B),  \label{eqn:recon}
% \end{aligned}
% \end{equation} 
\begin{equation}
\begin{aligned}
&\mathcal{L}_{t}^{\text{CSSL}}(\{\bm x^A, \bm x^B\};\bm \theta_t, \bm \theta_{t-1})\\ 
&=
\mathcal{L}^{\text{SSL}^*}_1(\{\bm z_t^A, \bm z_t^B, \bm z_{t-1}^A, \bm z_{t-1}^B\})\\&+  \mathcal{L}^{\text{SSL}^*}_2(\{g(\bm z_t^A), \bm z_{t-1}^A, \bm z_{t-1}^B, \bm z_t^A, \bm z_t^B\}).  
\end{aligned}\label{eqn:cont_form}
\end{equation} 
\csmcm{Here, $g(\cdot)$ represents another MLP layer (referred to as the Predictor in the figure) introduced in \cite{(cassle)fini2022self}, which has the same shape as $m_{\bm \psi_{t}}$.}
The SSL loss function $\mathcal{L}_{1/2}^{\text{SSL}^{*}}$ are newly designed general loss forms incorporating all candidate pseudo-negatives: $\bm z_{t-1}^A, \bm z_{t-1}^B$ for $\mathcal{L}^{\text{SSL}^{*}}_1$ and $\bm z_t^A, \bm z_t^B$ for $\mathcal{L}^{\text{SSL}^{*}}_2$. They resemble the two loss functions utilized in CaSSLe, and we will highlight the specific difference later. Furthermore, in order to 
\csmcm{consider two different augmentations in a symmetric fashion, we employ the following average as the final loss function for our method $\frac{1}{2}(\mathcal{L}_{t}^{\text{CSSL}}(\bm x^A, \bm x^B) + \mathcal{L}_{t}^{\text{CSSL}}(\bm x^B, \bm x^A))$.}
% The overall loss for CSSL is symmetric, such as $\frac{1}{2}(\mathcal{L}_{t}^{\text{CSSL}}(\bm x^A, \bm x^B) + \mathcal{L}_{t}^{\text{CSSL}}(\bm x^B, \bm x^A))$.

\begin{figure}[t]
\vspace{-.05in}
\centering 
{\includegraphics[width=0.98\linewidth]{figures/new_fig2.pdf}}
\vspace{-.2in}
\caption{Graphical representation of learning with our proposed loss. The blue dashed arrow indicates the direction of the gradient update during training with the proposed loss. It moves away from the negative and pseudo-negative embeddings, which correspond to current and past models, while converging towards the positive embeddings of the current and past models.}
\vspace{-.15in}
\label{figure:illustration}
 \end{figure}

 
As mentioned above, CaSSLe also uses two SSL loss functions, one responsible for plasticity and the other for stability, but they do not utilize any pseudo-negatives. Namely, the plasticity loss of CaSSLe (which corresponds to $\mathcal{L}^{\text{SSL}^{*}}_1$ of ours) is designed to learn new representations from the new task $t$ and only utilizes the output features from the current model $t$. Moreover, the stability loss of CaSSLe (which corresponds to $\mathcal{L}^{\text{SSL}^{*}}_2$ of ours) aims to maintain the representations learned from the past task $t-1$ and only regularizes with the output features from the previous model $t-1$.
% that the CaSSLe does not use the pseudo-negatives in both loss functions ($\mathcal{L}^{\text{SSL}^{*}}_1$ and $\mathcal{L}^{\text{SSL}^{*}}_2$) and leverages existing SSL methods to achieves plasticity and stability in CSSL.
% Specifically, for the identical anchor of the model $t$, the CaSSLe's $\mathcal{L}^{\text{SSL}^{*}}_1$ aims to learn new representations (\textit{i.g.}, plasticity) from the new task by minimizing the SSL loss through the sole use of positive and negative pairs from output features from the model $t$. 
% In contrast, the CaSSLe's $\mathcal{L}^{\text{SSL}^{*}}_2$ aims to maintain learned representations (\textit{i.g.}, stability) by employing positive and negative pairs from the output features of the model $t-1$.
We argue that such a stability loss term, designed to preserve representations from the previous model, might impede the plasticity loss, that aims to learn new representations from the new task but does not consider any representations from the previous model~\citep{(repeval)cha2023objective, kim2023stability}. 
% ability to learn new representation from the new task 
% improved representations when \csmcm{learning with} new task data~\citep{(repeval)cha2023objective, kim2023stability}. Moreover, the divergent configuration of positive and negative pairs for the same anchor could lead to conflicts in the learned representations, potentially hindering the acquisition of superior representations. 
To address these issues, we propose utilizing the output features of both the model $t-1$ and $t$ as the \textit{pseudo-negatives}, that can effectively work as regularizers so that the newly learned representations may not interfere with previously learned representations. 


% ensuring that each loss term learns representations from the same configuration of negatives.

In the upcoming section, we will specifically introduce novel function forms for $\mathcal{L}^{\text{SSL}^{*}}_1$ and $\mathcal{L}^{\text{SSL}^{*}}_2$ tailored to integrate pseudo-negatives into contrastive learning methods (e.g., SimCLR~\cite{(simclr)chen2020simple}, MoCo~\cite{(moco)he2020momentum}). Additionally, we will present how the idea of using pseudo-negatives can be applied to non-contrastive learning methods (e.g., BYOL~\cite{(byol)grill2020bootstrap}, VICReg~\cite{(vicreg)bardes2022vicreg}, BarlowTwins~\cite{(barlow_twins)zbontar2021barlow}) as well.

\subsection{InfoNCE-based Contrastive Learning Case}\label{sec:method_contrastive} 
Here, we propose new loss functions for CSSL using contrastive learning-based SSL methods (\textit{e.g.}. SimCLR and MoCo). First, $\mathcal{L}^{\text{SSL}^*}_1$ in (\ref{eqn:cont_form}) is defined as:
\begin{equation}
\begin{aligned}
&\mathcal{L}^{\text{SSL}^{*}}_1(\{\bm z_t^A, \bm z_t^B, \bm z_{t-1}^A, \bm z_{t-1}^B\})\\&=- {\mathrm{log}}\frac{\mathrm{exp}(\bm z^A_{t,i} \cdot \bm z^{B}_{t,i} / \tau)}{\sum_{\bm z_j\in\mathcal{N}_1(i)\cup\mathcal{PN}_1(i)}\exp (\bm z^A_{t,i}\cdot \bm z_j/\tau)},
\label{eqn:plasticity}
\end{aligned}
\end{equation} 
in which 
$\mathcal{N}_1(i)=\{\bm z_{t}^A, \bm z_{t}^B\}\backslash \{z_{t,i}^A\}$ is the set of original negatives,
% $\mathcal{N}(i)=\{\bm z_{t,k}^A\}_{k\neq i} \cup \bm z_{t,k}^B$ 
and
$\mathcal{PN}_1(i)=\{\bm z_{t-1}^A, \bm z_{t-1}^B\}\backslash \{z_{t-1,i}^A\}$ are pseudo-negatives of $\mathcal{L}^{\text{SSL}^{*}}_1$.
% $\mathcal{PN}(i)=\{\bm z_{t-1,k}^A\}_{k\neq i} \cup \bm z_{t-1,k}^B$. 
Also, $\mathcal{L}^{\text{SSL}^*}_2$ is defined as follows:
\begin{equation}
\begin{aligned}
&\mathcal{L}^{\text{SSL}^{*}}_2(\{g(\bm z_t^A), \bm z_{t-1}^A, \bm z_{t-1}^B, \bm z_t^A, \bm z_t^B\})\\&=- {\mathrm{log}}\frac{\mathrm{exp}(g(\bm z^A_{t,i}) \cdot \bm z^{A}_{t-1,i} / \tau)}{\sum_{\bm z_j\in\mathcal{N}_2(i)\cup\mathcal{PN}_2(i)}\exp (g(\bm z^A_{t,i})\cdot \bm z_j/\tau)},
\label{eqn:stability}
\end{aligned}
\end{equation} 
in which 
$\mathcal{N}_2(i)=\{\bm z_{t-1}^A, \bm z_{t-1}^B\}\backslash \{z_{t-1,i}^A\}$ is the original negatives for contrastive distillation~\cite{(cont_distill1)tian2019contrastive, (cassle)fini2022self},
% $\mathcal{N}(i)=\{\bm z_{t-1,k}^A\}_{k\neq i} \cup \bm z_{t-1,k}^B$ 
and 
$\mathcal{PN}_2(i)=\{\bm z_{t}^A, \bm z_{t}^B\}\backslash \{z_{t,i}^A\}$ is the pseudo-negatives of $\mathcal{L}^{\text{SSL}^{*}}_2$.
% $\mathcal{PN}(i)=\{\bm z_{t,k}^A\}_{k\neq i} \cup \bm z_{t,k}^B$. 
Also, $\tau$ denotes a temperature parameter.
% and $\mathrm{exp}$ stands for an exponential function. 
In the case of SimCLR, $\mathcal{N}_1(i)$, $\mathcal{PN}_1(i)$, $\mathcal{N}_2(i)$, and $\mathcal{PN}_2(i)$ consist of negatives from the current batch. When using MoCo, two queues storing positives of each loss function ($\mathcal{L}^{\text{SSL}^{*}}_1$ and $\mathcal{L}^{\text{SSL}^{*}}_2$) from previous iterations  are employed for them.

Note these two losses are quite similar in form to InfoNCE~\citep{(infonce)oord2018representation}, have has a couple of key differences. 
First, in $\mathcal{L}_{\text{1}}^{\text{SSL}^*}$, we use pseudo-negatives in $\mathcal{PN}_1(i)$ which are obtained from the previous model $h_{\bm \theta_{t-1}}$. 
This addition of negative embeddings in $\mathcal{L}_{\text{1}}^{\text{SSL}^*}$ compels the embedding of $\bm x_i$ to be repelled not only from the negative embeddings of the current model but also from those of the previous model, hence, it fosters the acquisition of more distinctive representations. 
Second, in $\mathcal{L}_{\text{2}}^{\text{SSL}^*}$, which has the similar form of contrastive distillation, we also use pseudo-negatives in $\mathcal{PN}_2(i)$. Such modification has the impact of placing additional constraints on distillation, ensuring that the representations from the past model are maintained in a way that does not contradict the representations of the current model.
% Also, we introduce the ``Predictor'' layer, as in \cite{(cassle)fini2022self}, to not hurt the plasticity by doing indirect distillation. 
Note that the denominators of the two loss functions are identical except for the $g(\cdot)$ in $\mathcal{L}_{\text{2}}^{\text{SSL}^*}$. 
Therefore, with the identical denominators, adding two losses will  result in achieving a natural trade-off between plasticity and stability for learning the representation. 

This intuition is depicted in the left figure of Figure \ref{figure:illustration}. Namely,  both losses symmetrically consider the embeddings from current and previous models, and as shown in the hypersphere, the representation of $\bm z^{A}_{t,i}$ gets attracted to $\bm z^{B}_{t,i}$ and $\bm z^{A}_{t-1,i}$ with the constraint that it is far from $\bm z^{B}_{t-1,i}$. Thus, the new representation will be distinctive from the previous model (\textit{plasticity}) and carry over the old knowledge (\textit{stability}) in a way not hurt the current model. 

The gradient analysis of the proposed loss function is detailed in Section \ref{sec:sup_gradient} of the Appendix.


 % \csm{It is noteworthy that the proposed loss can be easily integrated into contrastive learning-based SSL methods like MoCo and SimCLR. The implemented loss function for them is presented in the Supplementary Materials.}


% \noindent\textbf{Analysis of the gradients} \ \
% Here, we give the gradient analysis of our proposed loss for contrastive learning methods. For simplicity, we assume that ``\text{Pred}'' is an identity map instead of a MLP, hence $\tilde{z}_{i, t} = z_{i, t}$. Now, as given in the Supplementary Material, we can show the gradient of $\mathcal{L}_{\text{AugNeg}}$ with respect to $z_{i,t}$ becomes
% \begin{equation}
% \begin{aligned}
% &\scalemath{0.9}{\frac{\partial (\frac{1}{2}\mathcal{L}^{\text{CSSL}}_t(x_i))}{\partial z_{i,t}} = -\underbrace{\Bigg(\frac{z^{+}_{i,t} + z_{i,t-1}}{2}\Bigg)}_{(a)}} \\ &
% \scalemath{0.9}{+ \underbrace{\Bigg\{\sum_{z^{-}_{i,t}\in \mathcal{N}_t(i)} z^{-}_{i,t} \cdot M_{i,t}(z^{-}_{i,t}) + \sum_{z^{-}_{i,t-1}\in \mathcal{N}_{t-1}(i)} z^{-}_{i,t-1} \cdot M_{i,t}(z^{-}_{i,t-1})\Bigg\}}_{(b)},} \label{eqn:gradient}\ \ \ \nonumber
% \end{aligned}
% \end{equation}
% in which $M_{i,t}(u) = \mathrm{exp}(z_{i,t} \ \cdot \ u) / \big[S({z}_{i, t}, \mathcal{N}_t(i)) + S({z}_{i, t}, \mathcal{N}_{t-1}(i))\big]$, and $\sum_{z^{-}_{i,t}\in \mathcal{N}_t(i)}{M_{i,t}(z^{-}_{i,t})} + \sum_{z^{-}_{i,t-1}\in \mathcal{N}_{t-1}(i)}{M_{i,t}(z^{-}_{i,t-1})} = 1$. 
% Similarly as in the Unified Gradient of the InfoNCE loss \citep{(selfsup_analysis)tao2022exploring}, we can make the following interpretations. Namely, the negative gradient step can be decomposed into two parts, part (a) and the negative of part (b) above.


% Part (a) is the average of the embedding of $h_{\theta_t}$ for the positive sample and the embedding of $h_{\theta_{t-1}}$ for the input sample (\textit{i.e., }$x_i$). Hence, this direction encourages the model to learn new representations while taking the \textit{stability} from the previous model into account. On the other hand, negative of part (b) is the repelling direction from the center of mass point among the negative sample embeddings in $\mathcal{N}_t(i) \cup \mathcal{N}_{t-1}(i)$, in which each element $u\in\mathcal{N}_t(i) \cup \mathcal{N}_{t-1}(i)$ has the probability mass $S_{i,t}(u)$. Thus, this direction promotes the new representations to be more discriminative from the current and previous models' negative sample embeddings, leading to improved \textit{plasticity}. 
% Our gradient analysis allows us to better understand the graphical representation in the left figure of Figure \ref{figure:illustration}.



\subsection{Non-Contrastive Learning Case}\label{sec:method_non_contrastive}

\csm{Non-contrastive learning methods, such as Barlow, BYOL, and VICReg, do not incorporate negative samples. Therefore, the direct application of pseudo-negatives used for contrastive learning methods is not viable for these methods. 
However, motivated by the configuration of negatives in Equation (\ref{eqn:stability}), we propose a novel regularization that considers the pseudo-negatives from a new perspective. 
To achieve this, we propose new formulations of $\mathcal{L}^{\text{SSL}^{*}}_1$ and $\mathcal{L}^{\text{SSL}^{*}}_2$, tailored for non-contrastive learning methods, as follows:}
\begin{equation}
\begin{aligned}
&\mathcal{L}^{\text{SSL}^{*}}_1(\{\bm z_t^A, \bm z_t^B, \bm z_{t-1}^A, \bm z_{t-1}^B\}) = \mathcal{L}^{\text{SSL}}(\{z_t^A, \bm z_t^B\}),
\end{aligned}\label{eqn:noncont_l2_1}
\end{equation} 
where $\mathcal{L}^{\text{SSL}}$ denotes a non-contrastive SSL loss, and
\begin{equation}
\begin{aligned}
&\mathcal{L}^{\text{SSL}^{*}}_2(\{g(\bm z_t^A), \bm z_{t-1}^A, \bm z_{t-1}^B, \bm z_t^A, \bm z_t^B\}) \\ &= \mathcal{L}^{\text{SSL}}(\{g(\bm z_t^A), \bm z_{t-1}^A\}) - \lambda *\sum_i \sum_{\bm z_j\in\mathcal{PN}_2(i)}\|g(\bm z_{t,i}^A) - \bm z_j\|^2_2,
\end{aligned}\label{eqn:noncont_l2_2}
\end{equation} 
where $\mathcal{PN}_2(i)=\{\bm z_{t-1,i}^B\}$ is the pseudo-negative, $\|\cdot\|^2_2$ represents the squared $L_2$ norm and $\lambda$ is a hyperparameter. Additionally, $\bm z_{t-1}^A$ and $\bm z_{t-1}^B$ of Equation (\ref{eqn:noncont_l2_1}), as well as $ \bm z_t^A$ and $\bm z_t^B$ of Equation (\ref{eqn:noncont_l2_2}), are not employed when using non-contrastive learning.

Note that $\mathcal{L}^{\text{SSL}}$ of Equation (\ref{eqn:noncont_l2_2}) is the CaSSLe's distillation \csmcm{for a non-contrstive learning method}, and we introduce a new regularization to incorporate the pseudo-negatives. Specifically, $\bm z_{t-1,i}^B$ is assigned as the pseudo-negative of $\bm z_{t,i}^A$ (the anchor). This assignment stems from the configuration of negatives of Equation (\ref{eqn:stability}).
For example, when implementing Equation (\ref{eqn:stability}) using SimCLR and $N$ is the mini-batch size, $\mathcal{N}(i)$ consists of $2N-1$ negatives excluding $z_{t-1,i}^A$. Consequently, for a given anchor $\bm z_{t,i}^A$, an output feature $\bm z_{t-1, i}^B$ from the same image $\bm x_i$ but subjected to different augmentation is naturally considered as a negative (this holds true when using MoCo). This leads to minimizing the similarity between $g(\bm z_{t,i}^A)$ and $\bm z_{t-1,i}^B$ for the training task $t$.
To apply this concept of negatives to CSSL using non-contrastive learning, we propose a novel regularization that maximizes the squared mean square error between $g(\bm z_{t,i}^A)$ and $\bm z_{t-1,i}^B$, ensuring their dissimilarity.


The right figure in Figure \ref{figure:illustration} illustrates   representation learning with pseudo-negative in CSSL using BYOL. The CaSSLe's representation learning relies on distinct update directions from each positive (e.g., $\bm z_{t}^A$ and $\bm z_{t-1}^A$) to achieve enhanced plasticity and stability, without taking negatives into consideration. 
However, incorporating the pseudo-negative enables the model to avoid conflicts in learning representations by considering the pseudo-negative from the model $t-1$—learning representations far from the pseudo-negative from the model $t-1$. Consequently, the model acquires more distinctive representations from the previous model (enhancing plasticity) while retaining prior knowledge (ensuring stability).
Note that Equation (\ref{eqn:noncont_l2_2}) can be applied in conjunction with various non-contrastive SSL methods. 
The implementation details \csmcm{for BYOL and VICReg} are provided in Section \ref{sec:implementation} of the Appendix.


We will refer to the overall framework of using pseudo-negatives for regularization in CSSL, applicable to both contrastive and non-contrastive learning as described above, as PNR (Pseudo-Negative Regularization).
% We will refer the overall framework of utilizing pseudo-negatives for regularization in CSSL as PNR (Pseudo-Negative Regularization). 

% Note that the Equation \ref{eqn:noncont_form} can be applied together with several non-contrastive SSL methods, such as BYOL, VICReg and BarlowTwins. 
% We believe that the above idea can similarly be applied to various SSL algorithms that do not explicitly involve negative samples through the addition of extra regularization. The implementation details for BYOL, VICReg and Barlow are introduced in the Supplementary Materials.

==> iclr2023/3_method_prev.tex <==
\vspace{-0.1in}
\section{Main Method}
\subsection{Problem Setting}\label{sec:setting}
\noindent\textbf{Notations and preliminaries.}  \ \
We evaluate the quality of CSSL methods using the setting and data for continual supervised learning similarly as in \cite{(cassle)fini2022self}. Namely, let $t$ be the task index, where $t \in \{1, \dots, T\}$, and $T$ represents the maximum number of tasks. The input data and their corresponding true labels given at the $t$-th task are denoted by $ x \in \mathcal{X}_t$ and $y \in \mathcal{Y}_t$, respectively\footnote{For concreteness, we explicitly work with image data in this paper, but we note that our method is general and not confined to image modality.}. 
We assume each training dataset for task $t$ comprises 
$M$ supervised pairs, denoted as $\mathcal{D}_t = \{ (x_i, y_i)\}^{M}_{i=1}$, in which each pair is considered to be sampled from a joint distribution $p(\mathcal{X}_t, \mathcal{Y}_t)$.
Note in the case of continual supervised learning (CSL)~\citep{(cl_survey2)delange2021continual, (cil_survey)masana2020class}, both inputs and the labels are used, whereas in CSSL~\citep{(cassle)fini2022self,(continuity)madaan2022representational}, only input data are utilized for training, while the true labels are used only for the evaluation of the learned representations, such as linear probing or $k$-NN evaluation~\citep{(cassle)fini2022self, (repeval)cha2023objective}. 
We denote $h_{\theta_t}$ as the representation encoder (with parameter $\theta_t$) learned after task $t$ by a CSSL method. To evaluate the quality of $h_{\theta_{t}}$ via linear probing, we consider a classifier $f_{\Theta_{t}}= o_{\phi_{t}}\circ h_{\theta_{t}}$, in which $\Theta_t=(\theta_t,\phi_t)$ and $o_{\phi_{t}}$ is the linear output layer (with parameter $\phi_t$) on top of $h_{\theta_{t}}$. Then, only $o_{\phi_{t}}$ is supervised trained (with frozen $h_{\theta_{t}}$) using all the training dataset $\mathcal{D}_{1:t}$, including the labels, and the accuracy of resulting $f_{\Theta_{t}}$ becomes the proxy for the represenation quality. 


\noindent\textbf{Class-/Data-/Domain-incremental learning.}  \ \
We consider the three scenarios of continual learning as outlined in \cite{(CL_scenarios)van2019three, (cl_survey3)wang2023comprehensive, (cassle)fini2022self}. We use $k$ and $j$ to denote arbitrary task numbers, where $k,j\in \{1,\ldots,T\}$ and $k \neq j$. 
The first category is the \textit{class-incremental learning} (Class-IL), in which the $t$-th task's dataset consists of a unique set of classes for the input data, namely, $p(\mathcal{X}_k)\neq p(\mathcal{X}_j)$ and $\mathcal{Y}_k \cap \mathcal{Y}_j = \varnothing$.
The second category is \textit{domain-incremental learning} (Domain-IL), in which each dataset $\mathcal{D}_t$ has the same set of true labels but with different distribution on $\mathcal{X}_t$, denoted as $p(\mathcal{X}_k)\neq p(\mathcal{X}_j)$ but $\mathcal{Y}_k = \mathcal{Y}_j$.
In other words, each dataset in Domain-IL contains input images sampled from a different domain, but the corresponding set of true labels is the same as for other tasks.
Finally, we consider \textit{data-incremental learning} (Data-IL), in which a set of input images $\mathcal{X}_t$ is sampled from a single distribution, $p(\mathcal{X}_k) = p(\mathcal{X}_j)$, but $\mathcal{Y}_k = \mathcal{Y}_j$. 
To implement the Data-IL scenario in our experiments, we shuffled the entire dataset (such as ImageNet-100) and divided it into $T$ disjoint datasets.




\subsection{Motivation}\label{sec:motivation}

\noindent\textbf{Conventional loss form of continual learning}  \ \ 
We first reconsider the loss form, illustrated in Figure \ref{figure1:general_loss}, which is commonly employed by many state-of-the-art continual learning (CL) methods, except in cases where exemplar memory is utilized. 
Namely, when learning task $t$ with a model parameter $\Theta_t$, the conventional loss has the form as follows:
\begin{equation}
\mathcal{L}^{t}_{\mathrm{CL}}(\mathcal{D}_t, \Theta_t, \Theta_{t-1}) = \mathcal{L}_{\mathrm{single}}(\mathcal{D}_t, \Theta_t) + \lambda\cdot\mathcal{L}_{\mathrm{reg}}(\mathcal{D}_t, \Theta_t, \Theta_{t-1}),\label{eqn:general_cl}
\end{equation}
in which $\Theta_{t-1}$ represents the frozen model trained up to task $t-1$ and $\lambda$ denotes a regularization parameter that controls appropriate trade-off between the two loss terms.
\csm{The term $\mathcal{L}_{\mathrm{single}}$ represents the typical loss function utilized in single-task learning, such as cross-entropy, supervised contrastive loss ~\citep{(sup_contrastive)khosla2020supervised} or self-supervised learning loss~\citep{(moco)he2020momentum}.} This term clearly promotes \textit{plasticity} for the new task (task $t$) since it depends only on the current model $\Theta_{t}$ and $\mathcal{D}_t$. In addition, $\mathcal{L}_{\mathrm{reg}}$ represents a regularization term that is dedicated to increase \textit{stability}. Namely, since $\Theta_{t-1}$ is considered to contain knowledge of the previous tasks' dataset (\textit{i.e.}, $\mathcal{D}_{1:t-1}$) in the weight parameters, $\mathcal{L}_{\mathrm{reg}}$ is solely designed to maintain that knowledge to reduce forgetting while training $\Theta_t$ in various ways: such as direct weight level-regularization~\citep{(ewc)kirkpatrick2017overcoming}, knowledge distillation~\citep{(lwf)li2017learning} from $\Theta_{t-1}$ to $\Theta_{t}$, and model expansion term~\citep{(der)yan2021dynamically}.
\csm{It's worth noting that recent works on CSSL~\citep{(stream)hu2022how, (cassle)fini2022self, (continuity)madaan2022representational} also adopt a similar loss formulation as (\ref{eqn:general_cl}). In particular, CaSSLe~\citep{(cassle)fini2022self}, the current state-of-the-art method, introduces a novel and effective $\mathcal{L}_{\text{reg}}$ that easily integrates with various self-supervised learning methods, effectively mitigating catastrophic forgetting in learned representations during CSSL.}
% , such as Moco \citep{(moco)he2020momentum}, SimCLR \citep{(simclr)chen2020simple}, BYOL~\citep{(byol)grill2020bootstrap}, and BarlowTwins \citep{(barlow_twins)zbontar2021barlow}, etc.

Nevertheless, we contend that the utilization of such a conventional loss form may impose limitations on the achievement of more successful CSSL. This stems from the fact that while $\mathcal{L}_{\text{reg}}$ contributes to the preservation of previously acquired representations and the reduction of forgetting  , it may impede the acquisition of new representations from novel tasks. Furthermore, recent empirical findings, as highlighted in studies such as \citep{(repeval)cha2023objective, davari2022probing}, suggest that prioritizing \textit{stability} through regularization ($\mathcal{L}_{\text{reg}}$) may not necessarily result in learning improved representations even when higher accuracy is attained, thereby supporting this proposition.


\begin{figure}[t]
\vspace{-.1in}
\centering 
\subfigure[Conventional loss form of CL]
{\includegraphics[width=0.34\linewidth]{figures/fig1_a.pdf}
\label{figure1:general_loss}}
\subfigure[Lack of diversity of negative samples in CSSL]
{\includegraphics[width=0.64\linewidth]{figures/fig1_b.pdf}
\label{figure1:diversity}}
\vspace{-.15in}
\caption{Illustrations of motivation for our work. 
(a) Many of the CL algorithms combine a loss dedicated to learning a single current task and a regularizer that penalizes the deviation of the current model from the past.  
(b): In CSSL, negative samples are solely mined from the current task's data, resulting in significantly decreasing diversity of negative samples than the case of the joint SSL.}
\label{figure:fig1}
\vspace{-.2in}
 \end{figure}

\noindent\textbf{Low diversity of negative samples in CSSL}  \ \ 
In contrast to the prevailing research trend in CSSL, we assert that CSSL faces a critical challenge stemming from the \textit{limited diversity of negative samples} when compared to joint self-supervised learning (Joint SSL). 
\csm{The importance of negative samples in self-supervised contrastive learning has been extensively acknowledged, with studies demonstrating the benefits of incorporating a substantial number of diverse negative samples ~\citep{(infonce)oord2018representation,(contrastive_analysis)wang2020understanding, (simclr)chen2020simple, (selfsup_analysis)tao2022exploring} and selecting hard negatives ~\citep{(cont_hard_neg1)robinson2020contrastive,(cont_hard_neg2)kalantidis2020hard}. However, the issue of negative samples in the CSSL has remained unexplored until now.} In this regard, Figure \ref{figure1:diversity} highlights a fundamental problem: while Joint SSL allows for diverse negative sample selection, CSSL tends to exhibit significantly reduced diversity. Given the importance of negative samples, we believe that this decrease in diversity can be a key reason why self-supervised contrastive learning algorithms often yield less effective representations in CSSL scenarios, especially in terms of \textit{plasticity}.


% \csm{To tackle these new challenges, we pioneer the use of additional negative representations from both the $t$ and $t-1$ models to enhance the quality of learned representations during CSSL. Furthermore, we propose a simple but novel idea to apply these negative representations, not only to contrastive learning methods that leverage negatives ~\citep{(simclr)chen2020simple, (moco)he2020momentum} but also to conventional SSL methods that do not use negatives~\citep{(barlow_twins)zbontar2021barlow, (byol)grill2020bootstrap, (vicreg)bardes2022vicreg}.}



\subsection{Augmenting Negative Representations for Contrastive Learning Methods}\label{sec:method_contrastive} \ 

\begin{figure*}[h]
\vspace{-.05in}
\centering 
{\includegraphics[width=0.98\linewidth]{figures/fig2.pdf}}
\vspace{-.05in}
\caption{\csm{Graphical representation of learning with our proposed AugNeg loss. The blue dashed arrow represents the direction of the gradient update when training with the AugNeg loss, repelling from the negative sample embeddings of current/past models and attracting to the positive sample embeddings of the current/past models.}}
\vspace{-.2in}
\label{figure:recon_loss}
 \end{figure*}
 
Motivated by the two issues raised in the previous section, we propose a new form of loss functions tailored for CSSL. First, recalling the notation in Section \ref{sec:setting}, we note that only the encoder $h_{\theta_t}$ is trained during CSSL. Then, our Augmented Negatives (AugNeg) loss, devised for contrastive learning-based methods,  for learning from task $t$ has the following form
\begin{equation}
\mathcal{L}^{t}_{\text{AugNeg}}(\mathcal{D}_t, \theta_{t}, \theta_{t-1}) = \mathcal{L}_{\text{1}}(\mathcal{D}_t, \theta_{t}, \theta_{t-1}) + \mathcal{L}_{\text{2}}(\mathcal{D}_t, \theta_{t}, \theta_{t-1}).\label{eqn:recon}
\end{equation} 
While we will specify the two loss functions shortly, here, notice the symmetric dependence of them on $(\mathcal{D}_t,\theta_t,\theta_{t-1})$, which is in contrast to (\ref{eqn:general_cl}). As we show below, such symmetry enables our loss to promote finding inherent trade-off between the plasticity and stability without explicit control of a hyperparameter. 

\noindent\textbf{Model-based augmentation of negative representations.}  \ \ 
To address the issue depicted in Figure \ref{figure1:diversity} and based on the format of Equation (\ref{eqn:recon}), we propose 
to make use of augmented negative representations obtained from the both current and previous models \csm{during training task $t$}.
For given input data $x_i$ and encoder $h_{\theta_t}$, we denote  $z_{i, t} = \text{Proj}(h_{\theta_t}({x}_i)) \in \mathcal{R}^{D_P}$ and $\tilde{z}_{i, t} = \text{Pred}(z_{i, t}) \in \mathcal{R}^{D_P}$ as the normalized embeddings for the encoder of task $t$, in which ``Proj'' and ``Pred'' are the Projection~\citep{(simclr)chen2020simple} and Prediction~\citep{(cassle)fini2022self} layers, consisting of a multi-layer perceptron (MLP), respectively. Furthermore, we denote $z^{+}_{i,t}$ and $z^{-}_{i,t}$ as the embedding (obtained by $h_{\theta_t}$) of the \textit{positive} and \textit{negative} sample corresponding to the given $x_{i}$, respectively, and $\mathcal{N}_t(i)$ as the set of the negative embeddings for $x_i$. Then, both losses in (\ref{eqn:recon}) for the sample $x_i$ are defined as 
\begin{equation}
\mathcal{L}_{\text{1}}(x_i,\theta_t,\theta_{t-1}) = - {\mathrm{log}}\frac{\mathrm{exp}(z_{i, t} \cdot z^{+}_{i,t} / \tau)}{\sum_{z^{-}_{i,t}\in \mathcal{N}_t(i)}{\mathrm{exp}(z_{i, t} \cdot z^{-}_{i,t} / \tau) + {\sum_{z^{-}_{i,t-1}\in \mathcal{N}_{t-1}(i)}\mathrm{exp}(z_{i, t} \cdot z^{-}_{i,t-1} / \tau)}}}
\label{eqn:plasticity},\nonumber
\end{equation} 
and
\begin{equation}
\mathcal{L}_{\text{2}}(x_i,\theta_t,\theta_{t-1}) = - {\mathrm{log}}\frac{\mathrm{exp}(\tilde{z}_{i, t} \cdot z_{i,t-1} / \tau)}{\sum_{z^{-}_{i,t}\in \mathcal{N}_t(i)}{\mathrm{exp}(\tilde{z}_{i, t} \cdot z^{-}_{i,t} / \tau) + {\sum_{z^{-}_{i,t-1}\in \mathcal{N}_{t-1}(i)}\mathrm{exp}(\tilde{z}_{i, t} \cdot z^{-}_{i,t-1} / \tau)}}}\label{eqn:stability}.\nonumber
\end{equation} 
in which $\tau$ is a temperature parameter. 

Note these two losses are quite similar in form to InfoNCE~\citep{(infonce)oord2018representation}, but has a couple of key differences. Previous CL research, such as CaSSLe, $z_{i,t-1}$ was solely utilized for distilling previous knowledge (for better \textit{stability}).
In contrast to them, 
firstly, in $\mathcal{L}_{\text{1}}$, we use \textit{additional} negative embeddings in $\mathcal{N}_{t-1}(i)$ which are obtained from the previous model $h_{\theta_{t-1}}$. 
This addition of negative embeddings in $\mathcal{L}_{\text{1}}$ mitigates the issue of decreasing diversity of negative samples pointed out in Section \ref{sec:motivation}. Moreover, it compels the embedding of $x_i$ to be repelled not only from the negative embeddings of the current model but also from those of the previous model, hence, it fosters the acquisition of more distinctive representations. Secondly, in $\mathcal{L}_{\text{2}}$, which has the similar form of self-supervised distillation ~\citep{(cont_distill2)fang2021seed,(cont_distill1)tian2019contrastive}, we also use \textit{additional} negative embeddings in $\mathcal{N}_t(i)$. Such modification has an impact of putting additional constraint in distillation so that the representations from the past model are maintained in a way not to contradict with the representations of current model. Also, we introduce the ``Pred'' layer, as in \cite{(cassle)fini2022self}, to not hurt the plasticity by doing indirect distillation. 

Note that the denominators of the two loss functions are identical except for the ``Pred'' step in $\mathcal{L}_{\text{2}}$. 
Therefore, with the identical repelling negative embeddings, adding two losses will  result in achieving natural trade-off between plasticity and stability for learning the representation $z_{i,t}$. This intuition is depicted in Figure \ref{figure:recon_loss}. Namely, unlike in Figure \ref{figure1:general_loss}, both losses symmetrically consider the embeddings from current and previous models, and as shown in the rightmost hypersphere, the representation of $z_{i,t}$ gets attracted to $z_{i,t}^{+}$ and $z_{i,t-1}$ with the constraint that it is far from both $z_{i,t}^-$ and $z_{i,t-1}^-$. Thus, the new representation will be distinctive from the previous model (\textit{plasticity}) and carry over the old knowledge (\textit{stability}) in a way not to hurt the current model. 

 \csm{It is noteworthy that the AugNeg loss can be easily integrated into contrastive learning-based SSL methods like MoCo and SimCLR. The implemented loss function for them is presented in the Supplementary Materials. Also, 
in the Supplementary Materials, we provide more discussions and analyses, such as the gradient analysis for the proposed loss $\mathcal{L}_{\text{AugNeg}}$, the role of augmented negatives.}


\subsection{Extension to the Non-Contrastive Learning Methods}\label{sec:method_non_contrastive}
\csm{For SSL algorithms that do not utilize negatives (e.g., Barlow, BYOL and VICReg}), the core idea of AugNeg which utilizes model-based augmentation of negative representations cannot be directly applied.
However, we can apply the similar principle by adding an additional regularization term. For instance, consider a batch of input images denoted as \(x\), where distinct augmentations, denoted as \(A\) and \(B\), are applied, resulting in \(x^{A}\) and \(x^{B}\), respectively. 
Based on this, the loss function for the AugNeg loss s BYOL can be denoted as follows:
\begin{align}
\mathcal{L}^{t}_{\text{AugNeg, BYOL}}(x^{\text{A}}, x^{\text{B}}, \theta_{t}, \theta_{t-1}) = 
\|g_{\theta_t}(h_{\theta_t}(x^{\text{A}})) - {z_{\xi}}(x^{\text{B}})\|^2_2\label{eqn:byol} \\ +  
\|\text{Pred}(h_{\theta_t}(x^{\text{A}})) - h_{\theta_{t-1}}(x^{\text{A}})\|^2_2\label{eqn:cassle_byol} \\ -  
\|\text{Pred}(h_{\theta_t}(x^{\text{A}})) - h_{\theta_{t-1}}(x^{\text{B}})\|^2_2\label{eqn:augneg_byol}, 
\end{align}
where $q_{\theta_t}$ represents an MLP layer in BYOL, and $z_{\xi}$ corresponds to the target network obtained through momentum updates using $h_\theta$. 
Equation (\ref{eqn:byol}) and Equation (\ref{eqn:cassle_byol}) denotes the original loss function of BYOL and CaSSLe's distillation, respectively.
% Equation (\ref{eqn:byol}) maintains consistency with the self-supervised loss function used in the original BYOL. Equation (\ref{eqn:cassle_byol}) mirrors the approach employed in CaSSLe for distillation, which mitigates catastrophic forgetting in CSSL. 
Furthermore, \csm{Equation (\ref{eqn:augneg_byol}) is a newly devised regularization to enhance \textit{plasticity} by using negatives from the $t-1$ model.} Unlike Equation (\ref{eqn:cassle_byol}), where the outputs of models $t$ and $t-1$ task remain consistent when the same augmentation is applied, Equation (\ref{eqn:augneg_byol}) ensures that when different augmentations are applied, model $t$ produces different outputs from model $t-1$ (i.e., considering the output of model $t-1$ as negative samples). The justification for Equation (\ref{eqn:augneg_byol}) can be substantiated by the approach utilized in contrastive distillation of CaSSLe, where all samples with distinct augmentations (e.g., $2N$ samples) consider all samples except those with the same augmentation (e.g., $2N-1$ samples) as negative samples (See the Supplementary Materials for more details).
\csm{Note that the similar form of Equation \ref{eqn:augneg_byol} can be utilized for the case of AugNeg(VICReg) also. We believe that the above idea can similarly be applied to various SSL algorithms that do not explicitly involve negative samples through the addition of extra regularization. The implementation details for VICReg and Barlow are introduced in the Supplementary Materials.}

% where $q_{\theta_t}$ represents a MLP layer of BYOL, while $z_{\xi}$ corresponds to the target network obtained through momentum updates using $h_\theta$. 
% Equation (3) remains consistent with the self-supervised loss function employed in the original BYOL. 
% Equation (4) mirrors the implementation of CaSSLe~\cite{(cassle)fini2022self}'s distillation, which is employed to mitigate catastrophic forgetting in CSSL. Furthermore, Equation (5) introduces an additional regularization term. Unlike Equation (4), where the outputs of models $t$ and $t-1$ task remain consistent when the same augmentation is applied, Equation (5) ensures that, when different augmentations are applied, the model $t$ produces different outputs from the model $t-1$ (i.e., taking into account the output of the $t-1$ model as negative samples). 
% Also, the justification for Equation (5) can be substantiated by the approach utilized in CaSSLe for contrastive distillation between model t and t-1, where  considering all samples, except those with the same augmentation (e.g., 2N-1) as negative samples among all samples with distinct augmentations (e.g., 2N samples). 

% Similarly, we believe that our idea can be applied to various SSL algorithms that do not explicitly consider negative samples in the form of additional regularization. The implementation details of BarlowTwins are available in the Supplementary Materials. 

% \subsection{Discussion: the Role of Augmented Negative Representations}
% Incorporating augmented negative representations from the previous model (referred to as the $t-1$ model) aligns with SSL algorithms such as BYOL and MoCo, which leverage positive representations from a momentum encoder. This momentum encoder progressively enhances their representations by assimilating updates from the training encoder, thus contributing to the successful \textit{positive} representations for SSL. In contrast, in CSSL, the current task model (typically initialized as the $t-1$ model) is trained by leveraging information from the previous model. It's important to note that, while the previous model may have achieved adequate uniformity and alignment for the previous task dataset~\cite{(contrastive_analysis)wang2020understanding}, it may not exhibit the same characteristics when applied to a new task, as shown in Figure \ref{figure:recon_loss}. Therefore, in scenarios involving knowledge distillation (similar to CaSSLe~\cite{(cassle)fini2022self}), merely distilling the representations of samples from the current task dataset, such as representations of the same image with the same augmentation (\textit{e.g.}, Equation (4) and the numerator of $L_2$) may have a limitation to achieve a superior representation.

% In this regard, using augmented negative representations from the previous model can be considered as contributing to the informative additional \textit{negative} representations for CSSL. By additionally incorporating representations from both the models (\textit{e.g.,} the denominator of $L_1$ and $L_2$) or the previous model (\textit{e.g.,} Equation (5)) as supplementary negative representations, the newly trained model can learn superior and novel representations, taking into account both uniformity and alignment of not only the current but also previous model.



==> iclr2023/4_experiment.tex <==
\section{Experiments}

\subsection{Experimental Details}
\textbf{\noindent{Baselines}} \ \
To evaluate the proposed PNR, we set CaSSLe~\citep{(cassle)fini2022self} as our primary baseline, which has shown state-of-the-art performance in CSSL.
{We select five SSL methods, SimCLR~\citep{(simclr)chen2020simple}, MoCo v2 Plus (MoCo)~\citep{(mocov2)chen2020improved}, BarlowTwins (Barlow)~\citep{(barlow_twins)zbontar2021barlow},  BYOL~\citep{(byol)grill2020bootstrap}, and VICReg~\citep{(vicreg)bardes2022vicreg},  which achieve superior performance  with the combination with CaSSLe.}
% CaSSLe was applied to four SSL techniques: SimCLR~\citep{(simclr)chen2020simple}, MoCo v2 Plus (MoCo)~\citep{(mocov2)chen2020improved}, BarlowTwins (Barlow)~\citep{(barlow_twins)zbontar2021barlow}, and BYOL~\citep{(byol)grill2020bootstrap}. We ran their original code provided by CaSSLe without any modifications to the algorithms or their default hyperparameters. Additional details on baseline training settings can be found in the Supplementary Material.
% In order to evaluate the proposed Sy-CON loss, we have selected CaSSLe~\cite{(cassle)fini2022self} as our primary baseline, which has demonstrated state-of-the-art performance in CSSL. We present the results obtained by applying CaSSLe to four self-supervised learning techniques, including SimCLR~\cite{(simclr)chen2020simple}, MoCo v2 Plus (MoCo)\cite{(mocov2)chen2020improved}, BarlowTwins (BT)\cite{(barlow_twins)zbontar2021barlow}, and BYOL~\cite{(byol)grill2020bootstrap}, which have all exhibited superior performance with CaSSLe across various CSSL scenarios. The results are obtained by directly running their code proposed by CaSSLe, and no modifications were made to any of the algorithms or their default hyperparameters, except for the mini-batch size, which is set to the same value as Sy-CON, taking into account the hardware environment (see the implementation details section for more information). Additional details regarding the settings used to train the baseline are provided in the Supplementary Material.

\textbf{\noindent{Implementation details}} \ \
We implement our PNR based on the code provided by CaSSLe.
We conduct experiments on four datasets: CIFAR-100~\citep{(cifar)krizhevsky2009learning}, ImageNet-100~\citep{(imagenet)deng2009imagenet},  DomainNet~\citep{(domainnnet)peng2019moment}, and ImageNet-1k~\citep{(imagenet)deng2009imagenet} following the training and evaluation process outlined in \cite{(cassle)fini2022self}. For CIFAR-100 and ImageNet-100, we perform class- and data-incremental learning (Class- and Data-IL) for 5 and 10 tasks (denoted as 5T and 10T), respectively. For Domain-incremental learning (Domain-IL), we use DomainNet~\cite{(domainnnet)peng2019moment}, consisting of six disjoint datasets from different six source domains. 
Following experiments conducted by CaSSLe, we perform Domain-IL in the task order of "Real $\rightarrow$ QuickDraw $\rightarrow$ Painting $\rightarrow$ Sketch $\rightarrow$ InfoGraph $\rightarrow$ Clipart". Next, we report the average top-1 accuracy achieved by training a linear classifier separately for each domain, employing a frozen feature extractor (domain-aware evaluation).
% Due to time constraints, we only conduct experiments on Class-IL for 5T in the case of ImageNet-1000.
The ResNet-18~\citep{(resnet)he2016deep} model implemented in PyTorch is used except for ImageNet-1k where the ResNet-50 is employed. 
% {The proposed PNR is implemented based on the code provided by CaSSLe~\citep{(cassle)fini2022self}. 
% We conducted all experiments of both CaSSLe and PNR in the unified environment for fair comparison}. 
For all experiments except for ImageNet-1k, we perform each experiment using three random seeds and report the average performance across these trials.
Further experimental details are available in Section \ref{sec:details} of the Appendix.

% and the reported values represent the mean, with standard deviation indicated in parentheses (). 


% In order to conduct experiments in CSSL, we utilize three datasets, namely CIFAR-100~\cite{(cifar)krizhevsky2009learning}, ImageNet-100~\cite{(imagenet)deng2009imagenet}, and DomainNet~\cite{(domainnnet)peng2019moment}, following \cite{(cassle)fini2022self}. For CIFAR-100 and ImageNet-100, we perform Class- and Data-incremental learning (Class- and Data-IL) divided into 5 and 10 tasks, denoted by 5T and 10T, respectively. For Domain-incremental learning (Domain-IL), we utilize DomainNet, which consists of six disjoint datasets with different source domains. We use a ResNet-18 model~\cite{(resnet)he2016deep} implemented in Pytorch~\cite{(pytorch)NEURIPS2019_9015} for all experiments but modify the kernel size of the first layer to $3\times3$ only for experiments using CIFAR-100.
% The Sy-CON is implemented based on the code provided by CaSSLe~\cite{(cassle)fini2022self}, which is based on the solo-learn library~\cite{da2022solo}. The training settings for Sy-CON are identical to those used in CaSSLe with Barlow Twins, and we do not conduct an extensive hyperparameter search. The specific settings used in the experiments are as follows: 500, 400, and 200 epochs of training are performed for each task in experiments using CIFAR-100, ImageNet-100, and DomainNet datasets, respectively. A batch size of 256 is used for experiments using CIFAR-100, while a batch size of 128 is used for experiments using other datasets. Additionally, LARS~\cite{(lars)you2017large} is used for training in all experiments.
% All experiments were conducted on NVIDIA RTX A5000 with CUDA 11.2. We conduct each experiment three times with different seeds and reported the mean value, with the standard deviation indicated in parentheses ().
% Further details on the experimental settings can be found in the Supplementary Materials.


\textbf{\noindent{Evaluation metrics}} \ \
{To gauge the quality of representations learned in CSSL, we conduct linear evaluation by training only the output layer on the given dataset while maintaining the encoder $h_{\bm \theta_t}$ as a fixed component, following \citep{(cassle)fini2022self, (repeval)cha2023objective}}. 
The average accuracy after learning the task $t$ is denoted as {A$_{t}=\dfrac{1}{t}\sum_{i=1}^{T}a_{i,t}$}, where {$a_{i,j}$} stands for the linear evaluation top-1 accuracy of the encoder on the dataset of task $i$ after the end of learning task $j$.
Furthermore, we employ measures of stability ($S$) and plasticity ($P$), and a comprehensive explanation of these terms is provided in Section \ref{sec:measure} of the Appendix.


\begin{figure}[h]
\vspace{-.1in}
\centering
\includegraphics[width=0.9\linewidth]{iclr2023/figures/sycon_fig1.pdf}
\vspace*{-0.1in}
\caption{{Experimental results of applying PNR to SSL methods}. Note that "+CaSSLe" and "+PNR" indicate the results of applying CaSSLe and PNR to each SSL method, respectively.}\label{fig:applying}
\vspace{-.1in}
 \end{figure}
 
\subsection{Experiments with SSL Methods}

To assess the effectiveness of PNR when applied to various SSL methods, we conduct experiments by incorporating the PNR with MoCo, SimCLR, Barlow, BTOL, and VICReg, in the Class-IL (5T) scenario using CIFAR-100.
Figure \ref{fig:applying} illustrates that both the proposed PNR and CaSSLe are successfully combined with each SSL method, demonstrating progressively enhanced the quality of representations at each task.
However, PNR demonstrates more effective integration with MoCo, SimCLR, BYOL, {and VICReg}, surpassing the performance of CaSSLe.

% Firstly, when both CaSSLe and PNR are combined with each SSL method, they progressively enhance the quality of representations as each task $t$ is learned. Secondly, PNR demonstrates more effective integration with MoCo, SimCLR, BYOL, {and VICReg}, surpassing the performance of CaSSLe, which is the previous state-of-the-art method.

\begin{table}[h]
\vspace{-.1in}
\caption{{Experimental results of applying PNR to SSL methods in Class-IL (5T) with CIFAR-100. The * symbol indicates results from the CaSSLe paper, while the others are reproduced performance. The values in parentheses indicate the standard deviation and the \textbf{bolded} result represents the best performance.}}
% \vspace{-.15in}
\centering
\smallskip\noindent
% \vspace{-.1in}
\resizebox{.98\linewidth}{!}{
\begin{tabular}{c||c|c|c|c|c}
\hline
A$_{5}$        & MoCo                                                         & SimCLR                                                          & Barlow                                                          & BYOL & {VICReg}                                                            \\ \hline \hline
Joint          & \begin{tabular}[c]{@{}c@{}}66.90\\ (0.11)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}63.78\\ (0.22)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}68.99\\ (0.21)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}69.36\\ (0.28)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}68.01\\ (0.36)\end{tabular}       \\ \hline \hline
FT             & \begin{tabular}[c]{@{}c@{}}51.95\\ (0.26)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}48.97\\ (0.74)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}55.81\\ (0.57)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}52.43\\ (0.62)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}52.43\\ (0.62)\end{tabular}         \\ \hline
EWC*           & -                                                               & 53.60                                                           & 56.70                                                           & 56.40                                                       & -                                                           \\ \hline
DER*           & -                                                               & 50.70                                                           & 55.30                                                           & 54.80                                                         & -                                                           \\ \hline
LUMP*          & -                                                               & 52.30                                                           & 57.80                                                           & 56.40                                                         & -                                                           \\ \hline
Less-Forget*   & -                                                               & 52.50                                                           & 56.40                                                           & 58.60                                                        & -                                                           \\ \hline  
+CaSSLe         & \begin{tabular}[c]{@{}c@{}}60.11\\ (0.30)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}57.73\\ (1.07)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}60.10\\ (0.38)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}61.36\\ (1.38)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}53.13\\ (0.64)\end{tabular}          \\ \hline \hline
{+PNR} & {\begin{tabular}[c]{@{}c@{}}\textbf{62.36}\\ (0.29)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{58.87}\\ (0.16)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{60.28}\\ (0.36)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{63.19}\\ (0.39)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}\textbf{56.47}\\ (0.94)\end{tabular}} \\ \hline
\end{tabular}\label{fig:baseline_cifar100}
}
\vspace{-.1in}
\end{table}

% \begin{figure}[h]
% \vspace*{-0.1in}
% \begin{minipage}[b]{0.47\textwidth}
% \centering
% \includegraphics[width=0.98\textwidth]{iclr2023/figures/sycon_fig1.pdf}
% \vspace*{-0.1in}
% \caption{{Applying  PNR to SSL methods}.}\label{fig:applying}
% % \hfill
% \end{minipage}
% \begin{minipage}[b]{0.52\textwidth}
% \centering
% \resizebox{.98\linewidth}{!}{
%     \begin{tabular}{c||c|c|c|c|c}
% \hline
% A$_{5}$        & MoCo                                                         & SimCLR                                                          & Barlow                                                          & BYOL & {VICReg}                                                            \\ \hline \hline
% Joint          & \begin{tabular}[c]{@{}c@{}}66.90\\ (0.11)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}63.78\\ (0.22)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}68.99\\ (0.21)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}69.36\\ (0.28)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}68.01\\ (0.36)\end{tabular}       \\ \hline \hline
% FT             & \begin{tabular}[c]{@{}c@{}}51.95\\ (0.26)\end{tabular}           & \begin{tabular}[c]{@{}c@{}}48.97\\ (0.74)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}55.81\\ (0.57)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}52.43\\ (0.62)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}52.43\\ (0.62)\end{tabular}         \\ \hline
% EWC*           & -                                                               & 53.60                                                           & 56.70                                                           & -                                                       & 56.40                                                           \\ \hline
% DER*           & -                                                               & 50.70                                                           & 55.30                                                           & -                                                         & 54.80                                                           \\ \hline
% LUMP*          & -                                                               & 52.30                                                           & 57.80                                                           & -                                                         & 56.40                                                           \\ \hline
% Less-Forget*   & -                                                               & 52.50                                                           & 56.40                                                           & -                                                        & 58.60                                                           \\ \hline  
% CaSSLe         & \begin{tabular}[c]{@{}c@{}}60.11\\ (0.30)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}57.73\\ (1.07)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}60.10\\ (0.38)\end{tabular}          & \begin{tabular}[c]{@{}c@{}}61.36\\ (1.38)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}53.13\\ (0.04)\end{tabular}          \\ \hline \hline
% { PNR} & {\begin{tabular}[c]{@{}c@{}}62.36\\ (0.29)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}58.87\\ (0.16)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}60.28\\ (0.36)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}62.32\\ (0.98)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}56.47\\ (0.94)\end{tabular}} \\ \hline
% \end{tabular}
% }
% \vspace*{0.2in}
% \captionof{table}{{Experimental results on CSSL baselines.}}\label{fig:baseline_cifar100}
% \end{minipage}
% % \begin{minipage}[b]{0.29\textwidth}
% % \centering
% % \includegraphics[width=0.98\textwidth]{figures/recon_exp_fig2.pdf}
% % \caption{The graph of A$_{t}$}\label{fig:graph_cifar100}
% % \end{minipage}
% \vspace{-.1in}
% \end{figure}

Table \ref{fig:baseline_cifar100} presents the numerical results of $A_{5}$ in the same scenario. In this table, "Joint" corresponds to the experimental results in the Joint SSL scenario (upper bound) and "FT" represents the results achieved through fine-tuning with the SSL method alone. 
The table reveals that PNR consistently outperforms CaSSLe, showcasing a maximum improvement of approximately 2-3\%. 
Note that the extra performance gain achieved by PNR is particularly noteworthy, especially considering that CaSSLe's performance with MoCo, SimCLR, and BYOL is already close to that of the Joint.
% Especially notable is the additional performance improvement offered by PNR, particularly when taking into account the superior performance of CaSSLe with MoCo and BYOL, which is already approaching that of the Joint. 
% We contend that the extra performance improvement achieved by PNR is a noteworthy outcome.

% {Finally, Table \ref{table:forgetting_forward} presents stability ($S$) and plasticity ($P$) metrics. For MoCo, SimCLR, BYOL, and {VICReg}, the results illustrate PNR's superiority, attributed to a significant boost in \textit{plasticity} while minimizing increase of \textit{stability} compared to CaSSLe. This underscores the crucial role of employing the proposed model-based augmentation of negatives in CSSL.

% \begin{table}[h]
% \vspace{-.2in}
% \caption{Experimental results on stability and plasticity.}
% % \vspace{-.1in}
% \label{table:forgetting_forward}
% \centering
% \smallskip\noindent
% \resizebox{.98\linewidth}{!}{
% \begin{tabular}{|c||c|c|c|c|}
% \hline
% {$S(\downarrow)$ / $P(\uparrow)$}   & MoCo        & SimCLR      & BYOL      & {VICReg}         \\ \hline \hline
% CaSSLe & 0.11 / 9.99 & 0.33 / 4.08 & 0.09 / 11.94 & 0.39 / 6.78 \\ \hline
%  PNR   & 0.06 / 11.8 & 0.48 / 5.36 & 0.20 / 13.84 & 0.65 / 12.59 \\ \hline
% \end{tabular}
% }
% \vspace{-.1in}
% \end{table}

% Based on the results of these previous experiments, we will more focus to apply and evaluate  PNR(MoCo) and  PNR(BYOL), which achieves superior performance, in further experiments on various CSSL scenarios.}


\subsection{Experiments with Diverse CSSL Scenarios}
% \vspace{-.1in}
\begin{table}[t]
\caption{{The experimental results of Class-IL. All results are reproduced performance. The values in parentheses indicate the standard deviation and the \textbf{bolded} result represents the best performance.}}
% \vspace{-.15in}
\centering
\smallskip\noindent
% \vspace{-.1in}
\resizebox{.98\linewidth}{!}{
\begin{tabular}{|cc||ccc|}
\hline
\multicolumn{2}{|c||}{}                                         & \multicolumn{3}{|c|}{Class-IL}                                                                                                               \\ \cline{3-5} 
\multicolumn{2}{|c||}{}                                         & \multicolumn{1}{|c|}{CIFAR-100}                           & \multicolumn{2}{c|}{ImageNet-100}                                                \\ \cline{3-5} 
\multicolumn{2}{|c||}{\multirow{-3}{*}{A$_{T}$}}                & \multicolumn{1}{c|}{10T}                                 & \multicolumn{1}{c|}{5T}                                  & 10T                   \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{1}{c|}{66.90 (0.11)}                        & \multicolumn{2}{c|}{76.67 (0.56)}                                                \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{34.11 (0.90)}                        & \multicolumn{1}{c|}{57.87 (0.49)}                        & 47.48 (0.42)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{53.58 (0.41)}                        & \multicolumn{1}{c|}{63.49 (0.44)}                        & 52.71 (0.47)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{MoCo}}   & {+PNR} & \multicolumn{1}{c|}{{\textbf{56.62} (0.31)}}               & \multicolumn{1}{c|}{{\textbf{67.85} (0.44)}}               & {\textbf{60.75} (0.39)} \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{1}{c|}{63.78 (0.22)}                        & \multicolumn{2}{c|}{71.91 (0.57)}                                                \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{39.48 (1.00)}                        & \multicolumn{1}{c|}{56.11 (0.57)}                        & 46.66 (0.59)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{53.02 (0.47)}                        & \multicolumn{1}{c|}{62.53 (0.11)}                        & 54.55 (0.12)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{SimCLR}} & {+PNR} & \multicolumn{1}{c|}{{\textbf{53.47} (0.33)}}               & \multicolumn{1}{c|}{{\textbf{62.88} (0.19)}}               & {\textbf{54.79} (0.11)} \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{1}{c|}{69.36 (0.21)}                        & \multicolumn{2}{c|}{75.89 (0.22)}                                                \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{49.46 (0.67)}                        & \multicolumn{1}{c|}{60.27 (0.27)}                        & 51.83 (0.46)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{54.46 (0.24)}                        & \multicolumn{1}{c|}{{64.98 (0.79)}} & 56.27 (0.63)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{Barlow}} & {+PNR} & \multicolumn{1}{c|}{{\textbf{54.69} (0.21)}}               & \multicolumn{1}{c|}{{\textbf{65.38} (0.81)}}               & {\textbf{56.54} (0.42)} \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{1}{c|}{68.99 (0.28)}                        & \multicolumn{2}{c|}{75.52 (0.17)}                                                \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{46.13 (0.88)}                        & \multicolumn{1}{c|}{60.77 (0.62)}                        & 51.04 (0.52)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{{57.36 (0.86)}} & \multicolumn{1}{c|}{62.31 (0.09)}                        & 57.47 (0.75)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{BYOL}}   & {+PNR} & \multicolumn{1}{c|}{{\textbf{59.29} (0.25)}}               & \multicolumn{1}{c|}{{\textbf{64.23} (0.37)}}               & {\textbf{60.11} (0.91)} \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{1}{c|}{68.01 (0.36)}                        & \multicolumn{2}{c|}{75.08}                                                       \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{46.88 (0.28)}                        & \multicolumn{1}{c|}{55.58 (0.22)}                        &       \multicolumn{1}{c|}{46.88 (0.34)}                 \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{47.76 (0.46)}                        & \multicolumn{1}{c|}{59.18 (0.36)}                        & 49.98 (0.53)          \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{VICReg}} & {+PNR} & \multicolumn{1}{c|}{{\textbf{49.56} (0.56)}}               & \multicolumn{1}{c|}{{\textbf{62.48} (0.44)}}               & {\textbf{51.82} (0.50)} \\ \hline
\end{tabular}\label{table:class_il}
}
\vspace{-.1in}
\end{table}

\textbf{\noindent{Class-IL}} \ \
Table \ref{table:class_il} presents the experimental results of Class-IL with the CIFAR-100 and ImageNet-100 datasets. The results for Class-IL with CIFAR-100 (5T) can be found in Table \ref{fig:baseline_cifar100}.
In comparison to the state-of-the-art method, CaSSLe, PNR demonstrates superior performance across all scenarios. Notably, the combination of PNR with MoCo, BYOL, and VICReg exhibits significantly improved performance compared to their combination with CaSSLe. 
For example, in the ImageNet-100 experiments, "MoCo + PNR," "BYOL + PNR," and "VICReg + PNR" achieve a substantial gain of approximately 2-6\%, surpassing their combination with CaSSLe. 
As a result, we can confirm that the combination of PNR with each SSL method achieves state-of-the-art performance in the Class-IL scenarios.

% We believe that these findings underscore the effectiveness of the proposed PNR in Class-IL scenarios.
% Compared to the previous state-of-the-art method, CaSSLe, PNR achieves superior performance in all scenarios.
% Especially, the combination of PNR with MoCo, BYOL and VICReg achieves significantly improved performance compared to their combination with CaSSLe. For instance, in the ImageNet-100 experiments, "MoCo + PNR", "BYOL + PNR" and "VICReg + PNR" achieve a substantial gain of approximately 2-6\%, surpassing their combination with CaSSLe and establishing themselves as the new state-of-the-art methods.
% We believe that these results demonstrate the effectiveness of the proposed PNR in the Class-IL scenarios.


% \begin{wraptable}{r}{5.cm}
\begin{table}[h]
\vspace{-.1in}
\caption{{The experimental results of Class-IL with ImageNet-1k. The \textbf{bolded} result represents the best performance and we report results for a single seed.}}
% \vspace{-.15in}
\centering
\smallskip\noindent
% \vspace{-.1in}
\resizebox{.73\linewidth}{!}{
\begin{tabular}{c||cc|cc}
\hline
                          & \multicolumn{2}{c|}{MoCo}                                                   & \multicolumn{2}{c}{BYOL}                                                   \\ \cline{2-5} 
\multirow{-2}{*}{A$_{T}$} & \multicolumn{1}{c|}{5T}                                    & 10T            & \multicolumn{1}{c|}{5T}                                    & 10T            \\ \hline \hline
Joint                     & \multicolumn{2}{c|}{60.62}                                                  & \multicolumn{2}{c}{69.46}                                                  \\ \hline
FT                        & \multicolumn{1}{c|}{48.33}                                 & 42.55          & \multicolumn{1}{c|}{60.76}                                 & 57.15          \\ \hline
+CaSSLe                   & \multicolumn{1}{c|}{50.57}                                 & 43.38          & \multicolumn{1}{c|}{{64.78}}          & 61.93          \\ \hline
+PNR                      & \multicolumn{1}{c|}{\textbf{56.87}} & \textbf{55.88} & \multicolumn{1}{c|}{ \textbf{66.12}} & \textbf{62.56} \\ \hline
\end{tabular}\label{table:class_il_imagenet_1000}
}
\vspace{-.1in}
% \end{wraptable}
\end{table}

\textbf{\noindent{Class-IL with ImageNet-1k}} \ \
Table \ref{table:class_il_imagenet_1000} presents 
the experimental results of the ImageNet-1k dataset in Class-IL (5T and 10T).
We only conduct experiments for MoCo and BYOL, both of which have shown superior performance in previous experiments. 
We train a model for each method using the same hyperparameters employed in Class-IL with the ImageNet-100 dataset.
The experimental results in the table highlight the notable performance improvement of PNR in CSSL using the large-scale dataset, evident in both contrastive (MoCo) and non-contrastive (BYOL) learning methods. 
% These experimental results not only demonstrate the successful application of our proposed PNR to CSSL using both contrastive and non-contrastive learning methods again but also show its successful application even when dealing with a large-scale dataset.


\begin{table}[h]
% \vspace{-.15in}
\caption{{The experimental results of Data and Domain-IL. All results are reproduced performance. The values in parentheses indicate the standard deviation and the \textbf{bolded} result represents the best performance.}}
% \vspace{-.15in}
\centering
\smallskip\noindent
% \vspace{-.1in}
\resizebox{.98\linewidth}{!}{
\begin{tabular}{|cc||cc|c|}
\hline
\multicolumn{2}{|c||}{}                                         & \multicolumn{2}{c|}{Data-IL}                                                                                                          & Domain-IL                                                         \\ \cline{3-5} 
\multicolumn{2}{|c||}{}                                         & \multicolumn{2}{c|}{ImageNet-100}                                                                                                     & DomainNet                                                         \\ \cline{3-5} 
\multicolumn{2}{|c||}{\multirow{-3}{*}{A$_{T}$}}                & \multicolumn{1}{c|}{5T}                                           & 10T                                                               & 6T                                                                \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{2}{c|}{76.67 (0.56)}                                                                                                     & 48.20 (0.30)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{65.51 (0.72)}                                 & 60.50 (0.92)                                                      & 36.48 (1.01)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{66.88 (0.32)}                                 & 59.72 (0.61)                                                      & 38.04 (0.24)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{MoCo}}   & {+PNR} & \multicolumn{1}{l|}{\textbf{69.98} (0.30)} & \multicolumn{1}{l|}{{{\textbf{67.83} (0.45)}}} & \multicolumn{1}{l|}{{\textbf{43.86} (0.17)}} \\ \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{2}{c|}{71.91 (0.57)}                                                                                                     & 48.50 (0.21)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{62.88 (0.30)}                                 & 56.47 (0.11)                                                      & 39.46 (0.20)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{66.05 (0.95)}                                 & 61.68 (0.38)                                                      & 45.96 (0.19)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{SimCLR}} & {+PNR} & \multicolumn{1}{c|}{{\textbf{66.93} (0.12)}}                        & {\textbf{62.04} (0.28)}                                             & {\textbf{46.37} (0.13)}                                             \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{2}{c|}{75.89 (0.22)}                                                                                                     &            49.50 (0.32)                                                       \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{66.47 (0.24)}                                 & 59.48 (1.33)                                                      & 41.87 (0.17)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{{69.24 (0.36)}}          & {63.12 (0.28)}                               & 48.49 (0.04)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{Barlow}} & {+PNR} & \multicolumn{1}{c|}{{\textbf{70.16} (0.40)}}                        & {\textbf{64.06} (0.33)}                                                         & {\textbf{48.90} (0.07)}                                                         \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{2}{c|}{75.52 (0.17)}                                                                                                     &          53.80 (0.24)                                                         \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{69.76 (0.45)}                                 & 61.39 (0.44)                                                      & 47.29 (0.08)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{{\textbf{66.22} (0.13)}}          & {\textbf{63.33} (0.19)}                               & { 51.52 (0.18)}                               \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{BYOL}}   & {+PNR} & \multicolumn{1}{l|}{{ {66.08 (0.15)}}} & \multicolumn{1}{l|}{{{63.10 (0.28)}}} & \multicolumn{1}{l|}{{ {\textbf{51.96} (0.08)}}} \\ \hline \hline
\multicolumn{1}{|c|}{}                         & Joint         & \multicolumn{2}{c|}{75.08 (0.14)}                                                                                                     &                 52.12 (0.17)                                                  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & FT            & \multicolumn{1}{c|}{64.02 (0.11)}                                 &      \multicolumn{1}{c|}{57.30 (0.09)}                                                             &   46.11 (0.14)                                                                \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                         & +CaSSLe       & \multicolumn{1}{c|}{67.18 (0.15)}                                 & 61.50 (0.21)                                                      & 48.82 (0.12)                                                      \\ \cline{2-5} 
\multicolumn{1}{|c|}{\multirow{-4}{*}{VICReg}} & {+PNR} & \multicolumn{1}{c|}{{\textbf{67.68} (0.12)}}                        & {\textbf{62.08} (0.20)}                                             & {\textbf{48.95} (0.15)}                                             \\ \hline
\end{tabular}\label{table:data_il}
}
\vspace{-.05in}
\end{table}


\textbf{\noindent{Data-IL and Domain-IL}} \ \
Table \ref{table:data_il} presents the experimental results in Data- and Domain-IL using the ImageNet-100 dataset. In the results of Data-IL, the combination with PNR consistently achieves state-of-the-art performance in most cases. 
It is noteworthy that our PNR successfully integrates with MoCo once again, showcasing superior or nearly superior performance compared to other SSL methods at 5T and 10T. 
For instance, the combination "MoCo + PNR" demonstrates a 3-8\% performance enhancement compared to its pairing with CaSSLe. 
A similar trend is observed in Domain-IL, where the combination of CaSSLe with SSL methods already demonstrates superior performance close to their respective Joint's performance. However, PNR surpasses this by achieving additional performance improvements, thus setting new standards for state-of-the-art performance.
In contrast, "BYOL + PNR" performs worse than "BYOL + CaSSLe" in the Data-IL scenario. This can be attributed to the unique characteristics of Data-IL, which include shuffling and evenly distributing the ImageNet-100 dataset among tasks, leading to minimal distribution disparities between them. 
Additional discussion on this topic is available in Section \ref{sec:suboptimal} of the Appendix.



% \textbf{\noindent{Data-IL}} \ \
% Table \ref{table:data_il} presents the experimental outcomes for Data-IL utilizing the ImageNet-100 dataset. In most cases, excluding BYOL, our PNR consistently demonstrates performance improvement. Notably, PNR synergizes effectively with MoCo, leading to "MoCo + PNR" achieving nearly state-of-the-art performance in Data-IL (5T) and outperforming the state-of-the-art method in Data-IL (10T), "BYOL + CaSSLe", by a considerable margin. Additionally, we observed that PNR combined with non-contrastive learning methods exhibits slightly enhanced performance compared to its counterpart using CaSSLe.
% Also, when BYOL is integrated with CaSSLe and PNR in Data-IL, suboptimal results are obtained, particularly in the 5T scenario. This could be attributed to the distinctive characteristics of Data-IL, which involves shuffling and evenly distributing the ImageNet-100 dataset among tasks, resulting in minimal distribution disparities between them. Further discussion on this aspect is provided in Section \ref{sec:suboptimal} of the Appendix.

% \textbf{\noindent{Domain-IL}} \ \ 
%  The experimental results for Domain-IL with the DomainNet dataset are presented in the right column of Table \ref{table:data_il}. It's worth noting that, with the exception of MoCo, CaSSLe's results are already quite close to those of Joint (upper bound). However, we observe that our PNR enables the encoder to learn further enhanced representations compared to CaSSLe in most cases, bringing it closer to the performance of the Joint.
% % Note that, unlike the Data-IL scenario, where the application of PNR to BYOL led to only marginal performance improvement, in the Domain-IL setting, this combination demonstrates superior performance, bringing it into closer alignment with that of the Joint. 
% Finally, we believe that the substantial performance improvement of "MoCo + PNR" over "MoCo + CaSSLe" is particularly noteworthy.
%  % This difference can be attributed to the distinct variations in input distribution evident for each task in the Domain-IL scenario using the DomainNet dataset. Consequently, the inclusion of pseudo negatives proves more beneficial in learning enhanced representations.

Additionally, we conducted all experiments using CaSSLe's code and were able to reproduce the CaSSLe's reported performance on CIFAR-100. However, despite various efforts, we could only achieve performance that was 4-6\% lower than the CaSSLe's reported performance in experiments using ImageNet-100 and DomainNet. More discussion regarding this matter is provided in Appendix \ref{sec:reproduce}.


% \textbf{\noindent{Challenges of reproducing CaSSLe's results}} \ \
% In our experiments, we utilized CaSSLe's official code, yet observed results that were consistently 4-6\% lower than those reported in the original paper, particularly for datasets such as ImageNet-100 and DomainNet. 
% % Notably, similar discrepancies were documented on the issues page of CaSSLe's official GitHub repository. 
% However, our comparative experiments involving CaSSLe and our proposed PNR were conducted within an identical environment. This allows us to highlight the superior performance of PNR, eliminating confounding factors typically associated with fair comparisons. 
% For more in-depth insights into this matter, refer to the Appendix, where we discuss this issue and present our attempts to reproduce the CaSSLe's original performance, presented in Section \ref{sec:reproduce}.


% \begin{figure}[h]
% \vspace{-.1in}
% \centering 
% {\includegraphics[width=0.45\linewidth]{figures/recon_exp_fig1.pdf}}
% \vspace{-.05in}
% \caption{}
% \vspace{-.2in}
% \label{figure:recon_loss}
%  \end{figure}

% \begin{table}[h]
% \caption{}
% \label{table:norm_layers}
% \centering
% \smallskip\noindent
% \vspace{-.2in}
% \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|cccc|cccc}
%     \toprule
%     \multirow{2}{*}{Method} & \multicolumn{4}{c|}{CIFAR-100 w/ ResNet-32} & \multicolumn{4}{c}{ImageNet-100 w/ ResNet-18}\\
%      & $A_f(\uparrow)$ & $A_a(\uparrow)$ & $F(\downarrow)$ & $A_l(\uparrow)$ & $A_f(\uparrow)$ & $A_a(\uparrow)$ & $F(\downarrow)$ & $A_l(\uparrow)$\\
%     %\midrule
%     %Joint? &  &  &  &  &  &  &  & \\
%     \midrule
%     BN & 35.41 & 53.88 & 43.48 & 78.79 & 39.40 & 59.60 & 48.02 & 87.42 \\ 
%     IN & 31.72 & 46.84 & 47.72 & 79.44 & 33.45 & 53.59 & 50.69 & 84.66 \\ 
%     GN & 31.26 & 44.53 & 44.01 & 75.27 & 28.83 & 47.79 & 49.79 & 79.19 \\
%     SN & 36.29 & 53.64 & 42.91 & 79.20 & 39.45 & 59.55 & 48.04 & 87.79 \\ 
%     BRN & 36.08 & 52.58 & 44.34 & 80.42 & 37.49 & 57.77 & 48.13 & 86.57 \\
%     \midrule
%     CN & 35.06 & 54.43 & 43.82 & 80.64 & 41.96 & 60.02 & 45.32 & 87.28 \\ 
%     CN$^{*}$ & 36.05 & 54.18 & 44.81 & {80.85} & 40.46 & 59.03  & 46.74 & 87.20 \\
%     \midrule
%     TBBN & {38.46} & {56.17} & {41.90} & 80.36 & {43.20} & {61.69} & {43.62} & {87.82} \\ 
%     \bottomrule
%     \end{tabular}
% }
% \end{table}

% \vspace{-.2in}


\begin{figure*}[t]
\vspace{-.1in}
\centering 
\subfigure[MoCo + PNR]
{\includegraphics[width=0.32\linewidth]{figures/recon_exp_fig4_3_1.pdf}\label{figure:analysis_moco_pnr}}
\subfigure[{MoCo + CaSSLe}]
{\includegraphics[width=0.32\linewidth]{figures/recon_exp_fig4_2_1.pdf}\label{figure:analysis_moco_cassle}}
\subfigure[{MoCo + FT}]
{\includegraphics[width=0.32\linewidth]{figures/recon_exp_fig4_1_1.pdf}\label{figure:analysis_moco_ft}}
\subfigure[BYOL + PNR]
{\includegraphics[width=0.32\linewidth]{figures/recon_exp_fig4_4.pdf}\label{figure:analysis_byol_pnr}}
\subfigure[{BYOL + CaSSLe}]
{\includegraphics[width=0.32\linewidth]{figures/recon_exp_fig4_5.pdf}\label{figure:analysis_byol_cassle}}
\subfigure[{BYOL + FT}]
{\includegraphics[width=0.32\linewidth]{figures/recon_exp_fig4_7.pdf}\label{figure:analysis_byol_ft}}
\vspace{-.1in}
\caption{{The graph illustrates the values of a$_{k,t}$ of each algorithm in the Class-IL (5T) scenario using the ImageNet-100 dataset. The measured stability ($S \downarrow$) and plasticity ($P \uparrow$) of each method are as follows: (a) $(S, P)=(1.23, 3.47)$, (b) $(S, P)=(2.80, 2.52)$, (c) $(S, P)=(3.13, 2.38)$, (d) $(S, P)=(0.4, -0.07)$, (e) $(S, P)=(1.5, -0.47)$, (f) $(S, P)=(4.9, 1.6)$.}}
\label{figure:each_task_graph}
\vspace{-.15in}
 \end{figure*}

\subsection{Experimental Analysis}


\textbf{\noindent{Analysis on plasticity and stability}} \ \ 
{Figure \ref{figure:each_task_graph} presents the experimental results of Class-IL (5T) using the ImageNet-100 dataset, showcasing graphs of {a$_{k,t}$} and {Avg(a$_{1:5,t}$)}. 
From Figure \ref{figure:analysis_moco_pnr} showing the result of "MoCo + PNR", we observe a general upward trend in a$_{k,t}$ across all tasks. Remarkably, the performance of the initial task (a$_{k=1,t}$) remains relatively stable and even exhibits slight improvement as subsequent tasks are learned. 
Conversely, the results depicted in Figures \ref{figure:analysis_moco_cassle} and \ref{figure:analysis_moco_ft} of "MoCo + CaSSLe" and "MoCo + FT" indicate that, while their Avg(a$_{1:5,t}$) gradually increases, certain task performances experience gradual declines (e.g., a$_{k=2,t}$ of "MoCo + CaSSLe" and most $k$ of "MoCo + FT"), showing suffering from catastrophic forgetting than "MoCo + PNR".
Furthermore, the numerical assessments of plasticity ($P$) and stability ($S$) of each algorithm, as presented in the caption of Figure \ref{figure:each_task_graph}, demonstrate that "MoCo + PNR" achieves its performance improvement through superior \textit{plasticity} and \textit{stability} compared to other baselines. 

% Figure \ref{figure:analysis_byol_pnr}, \ref{figure:analysis_byol_cassle} and \ref{figure:analysis_byol_ft} depict the results of the experimental analysis conducted on "PNR + BYOL", "BYOL + CaSSLe", and "BYOL + FT" in Class-IL (5T) experiments using the ImageNet-100 dataset. The trends observed here align with previous results. First, there is a gradual increase in their Avg(a$_{1:5,t}$). However, it is noteworthy that a$_{k=1,t}$, a$_{k=3,t}$ for "BYOL + CaSSLe" decrease across tasks. Similarly, "BYOL + FT" shows a degraded performance in most $k$. In contrast, the application of the proposed PNR not only maintains a$_{k=1,t}$ well but also results in a gradual increase in a$_{k=2,t}$ and a$_{k=4,t}$, suggesting that PNR surpasses "BYOL + CaSSLe" in terms of plasticity and stability. Also, The plasticity ($P$) and stability ($S$) measurements mentioned in the caption of Figure \ref{figure:each_task_graph} further substantiate these experimental results.
% These analyses not only underscore the effectiveness of incorporating the pseudo-negative but also provide additional evidence of our PNR's superior performance. 
% The corresponding analysis for other baselines is available in Section \ref{sec:analysis} of the Appendix.

Figures \ref{figure:analysis_byol_pnr}, \ref{figure:analysis_byol_cassle}, and \ref{figure:analysis_byol_ft} illustrate the results of our experimental analysis conducted on "PNR + BYOL," "BYOL + CaSSLe," and "BYOL + FT" in Class-IL (5T) experiments using the ImageNet-100 dataset. These findings align with previous results, showing a gradual increase in Avg(a$_{1:5,t}$). 
However, significant declines are seen in a$_{k=1,t}$ and a$_{k=3,t}$ for "BYOL + CaSSLe" across tasks, whereas "BYOL + FT" shows decreased performance in most $k$. In contrast, the application of our proposed PNR not only maintains a$_{k=1,t}$ effectively but also leads to a gradual increase in a$_{k=2,t}$ and a$_{k=4,t}$, indicating that our PNR outperforms "BYOL + CaSSLe" in terms of plasticity and stability. Additionally, the plasticity ($P$) and stability ($S$) measurements mentioned in the caption of Figure \ref{figure:each_task_graph} further support these experimental findings.

In conclusion, these analyses not only highlight the effectiveness of integrating the pseudo-negative but also provide further evidence of the superior performance of our PNR. Additional analysis for other baselines can be found in Section \ref{sec:analysis} of the Appendix.

% Figure \ref{figure:each_task_graph2} depicts the results of the experimental analysis conducted on "PNR + BYOL", "BYOL + CaSSLe", and "BYOL + FT" in Class-IL (5T) experiments using the ImageNet-100 dataset. The trends observed here align with those presented in the manuscript. Initially, there is a gradual increase in their Avg(a$_{1:5,t}$). However, it is noteworthy that a$_{k=1,t}$, a$_{k=3,t}$ for "BYOL + CaSSLe" decrease across tasks. Similarly, "BYOL + FT" experiences a decline in most $k$. In contrast, the application of the proposed PNR not only maintains a$_{k=1,t}$ but also results in a gradual increase in a$_{k=2,t}$ and a$_{k=4,t}$, suggesting that PNR surpasses "BYOL + CaSSLe" in terms of plasticity and stability. 



\textbf{\noindent{Analysis on the impact of pseudo-negatives}} \ \ Table \ref{table:queue_main} presents the experimental results for different queue sizes (\textit{i.e.}, the size of $\mathcal{PN}_1(i)$ and $\mathcal{PN}_2(i)$) in "MoCo + PNR". Note that the default queue size is 65536 for all previous experiments. We observe that performance remains relatively consistent when the queue size exceeds 16384. However, significant performance degradation is evident with reduced queue sizes (\textit{i.e.}, reduced pseudo-negatives), particularly at 256. Based on this result, we affirm that the superior performance of "MoCo + PNR" is attributed to the utilization of a large number of pseudo-negatives.


\begin{table}[h]
\vspace{-.1in}
\caption{Experiments with different queue sizes.}
\label{table:queue_main}
\centering
\smallskip\noindent
% \vspace{-.2in}
\resizebox{.98\linewidth}{!}{
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
Queue size & 256   & 512  & 2048  & 16384 & {{65536}} & 131072 \\ \hline \hline
A$_{5}$    & 61.03 & 61.68 & 61.90 & 62.10 & {{62.36}} & 62.01  \\ \hline
\end{tabular}
}
\vspace{-.05in}
\end{table}




% \vspace{-.1in}
% \begin{table}[h]
% \caption{{Experimental results on downstream tasks. The red annotation represents the highest performance, while the blue annotation indicates the second-highest performance.}}
% % \vspace{-.15in}
% \label{table:semi_supervised_learning}
% \centering
% \smallskip\noindent
% % \vspace{-.1in}
% \resizebox{.98\linewidth}{!}{
% \begin{tabular}{c|c||c|c|c|c||c|c}
% \hline
% Case                              & Data           & \begin{tabular}[c]{@{}c@{}}MoCo\\  + CaSSLe\end{tabular} & \begin{tabular}[c]{@{}c@{}}SimCLR\\  + CaSSLe\end{tabular} & \begin{tabular}[c]{@{}c@{}}Barlow\\  + CaSSLe\end{tabular} & \begin{tabular}[c]{@{}c@{}}BYOL\\  + CaSSLe\end{tabular} & \begin{tabular}[c]{@{}c@{}} { PNR}\\  {(MoCo)}\end{tabular} & \begin{tabular}[c]{@{}c@{}} { PNR}\\  {(BYOL)}\end{tabular} \\ \hline \hline
%                                   & 10\%           & 56.48                                                    & 55.16                                                      & 55.10                                                      & 54.22                                                    & {\color[HTML]{FE0000} 61.74}                           & {\color[HTML]{3531FF} 57.36}                           \\ \cline{2-8} 
% \multirow{-2}{*}{Semi-supervised} & 1\%            & 39.14                                                    & 40.86                                                      & {\color[HTML]{3531FF} 41.90}                               & 36.86                                                    & {\color[HTML]{FE0000} 46.48}                           & 40.82                                                  \\ \hline \hline
%                                   & Three datasets & 58.61                                                    & 56.73                                                      & 58.13                                                      & 61.35                                                    & {\color[HTML]{3531FF} 62.04}                           & {\color[HTML]{FE0000} 62.53}                           \\ \cline{2-8} 
% \multirow{-2}{*}{Downstream}      & Clipart        & 28.32                                                    & 34.68                                                      & 37.42                                                      & {\color[HTML]{3531FF} 38.98}                             & 38.86                                                  & {\color[HTML]{FE0000} 41.57}                           \\ \hline
% \end{tabular}
% }
% \vspace{-.1in}
% \end{table}

\begin{table*}[t]
\vspace{-.1in}
\caption{{Experimental results of semi-supervised learning and downstream tasks. "10\%" and "1\%" denote the percent of used supervised datasets for semi-supervised learning. Also, "CIL", "DIL", "DTs" and 
"Cli." means "Class-IL", "Data-IL", "Downstream Tasks" and "Clipart", respectively. The \textbf{bolded} result represents the best performance}}
% \vspace{-.15in}
\label{table:semi_supervised_learning}
\centering
\smallskip\noindent
% \vspace{-.1in}
\resizebox{.98\linewidth}{!}{
\begin{tabular}{|cc||c|c|c|c||c|c|}
\hline
\multicolumn{2}{|c|}{}                                & \begin{tabular}[c]{@{}c@{}}MoCo  + CaSSLe\end{tabular} & \begin{tabular}[c]{@{}c@{}}SimCLR  + CaSSLe\end{tabular} & \begin{tabular}[c]{@{}c@{}}Barlow  + CaSSLe\end{tabular} & \begin{tabular}[c]{@{}c@{}}BYOL  + CaSSLe\end{tabular} & {\begin{tabular}[c]{@{}c@{}}MoCo + PNR\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}BYOL + PNR\end{tabular}} \\ \hline \hline
\multicolumn{1}{|c|}{}                          & CIL & {56.48}                             & {55.16}                               & {55.10}                           & {54.22}                             & {{\textbf{61.74}}}                         & {{57.36}}                         \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\rotatebox{90}{10\%}}}    & DIL & {62.66}                             & {60.14}                               & {62.18}                           & {59.48}                             & {{\textbf{65.28}}}                         & {{58.04}}                         \\ \hline 
\multicolumn{1}{|c|}{}                          & CIL & {39.14}                             & {40.86}                               & {41.90}                           & {36.86}                             & {{\textbf{46.48}}}                         & {{40.82}}                         \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\rotatebox{90}{1\%}}}     & DIL & {51.04}                             & {49.72}                               & {54.10}                           & {46.06}                             & {{\textbf{54.88}}}                         & {{44.46}}                         \\ \hline \hline
\multicolumn{1}{|c|}{}                          & CIL & {58.61}                             & {56.73}                               & {58.13}                           & {61.35}                             & {{62.04}}                         & {{\textbf{62.53}}}                         \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\rotatebox{90}{DTs}}}   & DIL & {59.15}                             & {56.97}                               & {59.54}                           & {61.61}                             & {{\textbf{62.35}}}                         & {{61.95}}                         \\ \hline
\multicolumn{1}{|c|}{}                          & CIL & 28.32                                                    & 34.68                                                      & 37.42                                                  & 38.98                                                    & {38.86}                                                & {\textbf{41.57}}                                                \\ \cline{2-8} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\rotatebox{90}{Cli.}}} & DIL & 29.74                                                    & 34.17                                                      & 36.13                                                  & 37.04                                                    & {38.33}                                                & {\textbf{40.06}}                                                \\ \hline
\end{tabular}
}
\vspace{-.1in}
\end{table*}


\textbf{\noindent{Semi-supervised learning and downstream tasks}} \ \
To evaluate the quality of learned representations in a more diverse way, we conduct experiments in a semi-supervised scenario. Specifically, we consider a scenario where a linear classifier is only trained using only 1\% or 10\% of the entire supervised ImageNet-100 dataset. We evaluate each encoder trained in the Class-IL (5T) and Data-IL (5T) using the ImageNet-100 dataset. The experimental results are presented in the upper rows of Table \ref{table:semi_supervised_learning}. 
Notably, when compared to CaSSLe, applying PNR to both MoCo and BYOL yields approximately 3-6\% performance improvements in both 10\% and 1\%, showing new state-of-the-art performances.
The lower rows of Table \ref{table:semi_supervised_learning} present the results of linear evaluation for downstream tasks conducted on the same encoders. For the three datasets, we report the average accuracy of linear evaluation results on STL-10~\citep{(stl10)coates2011analysis}, CIFAR-10, and CIFAR-100~\citep{(cifar)krizhevsky2009learning} datasets. Additionally, we set Clipart within the DomainNet~\citep{(domainnnet)peng2019moment} dataset as the downstream task and report the results of linear evaluation using it. From these experimental results, we once again demonstrate that both "MoCo + PNR" and "BYOL + PNR" achieve performance improvements compared to the CaSSLe's performance. 

More detailed results and additional findings (e.g., experiments using the model trained in Class-IL (10T) and Data-IL (10T) are provided in Section \ref{sec:downstream} of the Appendix.


\textbf{\noindent{Computational cost}} \ \ 
Note both PNR and CaSSLe incur almost identical computational costs, except for "MoCo + PNR," which involves an additional queue to store negatives from the $t-1$ model. However, the memory size required for this additional queue is negligible.

\textbf{\noindent{Ablation study}} \ \
Table \ref{table:ablation_study} presents the results of the ablation study conducted on CIFAR-100 in the Class-IL (5T) scenario. The first row represents the performance of "MoCo + PNR" when all negatives are used. Cases 1 to 3 illustrate the results when one of pseudo-negatives, $\mathcal{PN}_1(i)$ and  $\mathcal{PN}_2(i)$ is excluded or when both are omitted.
The experimental results show that the absence of these negatives leads to a gradual decrease in performance, indicating that "MoCo + PNR" acquires superior representations by leveraging both the pseudo-negatives.
Specifically, when $\mathcal{PN}_2(i)$ is omitted, the performance degradation is more significant compared to when the negative from $\mathcal{PN}_1(i)$ is absent.
Moreover, the result of Case 4, where a queue size twice as large is used for "MoCo + CaSSLe", demonstrates that using the proposed pseudo-negatives is different from simply increasing the queue size. Note that ablation study for PNR with non-contrastive learning, such as BYOL and VICReg, can be confirmed by comparing the results of "+CaSSLe" and "+PNR" in Table \ref{fig:baseline_cifar100}, \ref{table:class_il}, \ref{table:class_il_imagenet_1000}, and \ref{table:data_il}.

\begin{table}[h]
\vspace{-.1in}
\caption{{Ablation study of "MoCo + PNR" in Class-IL (5T) using the ImageNet-100 dataset.}}
% \vspace{-.1in}
\centering
\smallskip\noindent
\resizebox{.98\linewidth}{!}{
\begin{tabular}{c||c|c|c|c||c}
\hline
       & \begin{tabular}[c]{@{}c@{}}$\mathcal{PN}_1(i)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\mathcal{PN}_2(i)$\end{tabular} & + CaSSLe & $|$queue$|$ $\times 2$ & A$_{5}$ \\ \hline \hline
PNR &          \cmark                                 &             \cmark                                  &      \xmark    &          \xmark          & 62.36        \\ \hline
Case 1 &           \xmark                                &                    \cmark                           &      \xmark    &     \xmark               & 61.26   \\ \hline
Case 2 &              \cmark                             &             \xmark                                  &     \xmark     &      \xmark              & 60.92   \\ \hline
Case 3 &                                 \xmark          &                             \xmark                  &       \xmark   &            \xmark        & 59.97   \\ \hline
Case 4 &                         \xmark                  &           \xmark                                    &    \cmark      &            \cmark        &  60.09  \\ \hline
\end{tabular}\label{table:ablation_study}
}
\vspace{-.in}
\end{table}

Moreover, we present further experimental results of applying PNR to supervised contrastive learning in Section \ref{sec:supcon} of the Appendix.


% \vspace{-.15in}
% \noindent{$\mathcal{L}_\mathrm{plasticity}$ with CasSSLe} \ \


% \noindent{Training cost} \ \



% \noindent{Representation analysis using CKA} \ \





==> iclr2023/5_concluding_remarks.tex <==
\section{Limitation and Future Work}
There are several limitations to our work. First, we focused on Continual Self-Supervised Learning (CSSL) with CNN-based architectures (e.g., ResNet). However, we believe that our proposed idea and loss function could be applied to CSSL using vision transformer-based models. Second, we only considered CSSL in the computer vision domain. Nonetheless, we believe that the concept of pseudo-negatives could be extended to CSSL in other domains, such as natural language processing. We defer these explorations to the future work.

\section{Concluding Remarks}

We present Pseudo-Negative Regularization (PNR), a simple yet novel method employing pseudo-negatives in Continual Self-Supervised Learning (CSSL). First, we highlight the limitations of the traditional CSSL loss formulation, which may impede the learning of superior representations when training a new task. To overcome this challenge, we propose considering the pseudo-negatives generated from both previous and current models in CSSL using contrastive learning methods. Furthermore, we expand the concept of PNR to non-contrastive learning methods by incorporating additional regularization. Through extensive experiments, we confirm that our PNR not only can be applied to self-supervised learning methods, but also achieves state-of-the-art performance with superior stability and plasticity.

% {We introduce the Pseudo-Negative Regularization (PNR), a simple but novel approach using pseudo negative in continual self-supervised learning (CSSL). Initially, we highlight the limitations of the traditional CSSL loss formulation, which may hinder learning better representations during training a new task. To address this challenge, we propose considering pseudo negative from both previous and current models for InfoNCE-based contrastive learning. Furthermore, we show that the idea of PNR can be extended to non-contrastive methods by adding extra regularization. Through extensive experiments, we observe that not only our PNR can be applied to various self-supervised learning methods but also achieves state-of-the-art performance with superior stability and plasticity.}



\newpage



\section*{Impact Statement}

This paper presents a Pseudo-Negative Regularization (PNR) framework designed to advance Continual Self-Supervised Learning (CSSL). By balancing the trade-off between plasticity and stability during CSSL, our work contributes to the development of more energy-efficient AI systems, supporting both environmental sustainability and technological progress. Furthermore, our framework paves the way for more adaptive AI applications across various sectors.

\section*{Acknowledgment}
This work was supported in part by the National Research Foundation of Korea (NRF) grant [No.2021R1A2C2007884] and by Institute of Information \& communications Technology Planning \& Evaluation (IITP) grants
[RS-2021-II211343, RS-2021-II212068, RS-2022-II220113,
RS-2022-II220959] funded by the Korean government (MSIT). It was also supported by AOARD Grant No. FA2386-23-1-4079 and SNU-Naver Hyperscale AI Center. 
% While there are various potential societal consequences of our work, none require specific highlighting here.

% \csmcm{The work was supported in part by NRF grant [2021R1A2C2007884, 2021M3E5D2A01024795], IITP grant [No.2021-0-01343, No.2021-0-02068, No.2022-0-00113, No.2022-0-00959] funded by the Korean government, and SNU-Naver Hyperscale AI Center.}

% \newpage


==> iclr2023/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

